Class-attribute Priors: Adapting Optimization to Heterogeneity and Fairness Objective

Modern classification problems exhibit heterogeneities across individual classes: Each class may have unique attributes, such as sample size, label quality, or predictability (easy vs difficult), and variable importance at test-time. Without care, these heterogeneities impede the learning process, most notably, when optimizing fairness objectives. Confirming this, under a gaussian mixture setting, we show that the optimal SVM classifier for balanced accuracy needs to be adaptive to the class attributes. This motivates us to propose CAP: An effective and general method that generates a class-specific learning strategy (e.g. hyperparameter) based on the attributes of that class. This way, optimization process better adapts to heterogeneities. CAP leads to substantial improvements over the naive approach of assigning separate hyperparameters to each class. We instantiate CAP for loss function design and post-hoc logit adjustment, with emphasis on label-imbalanced problems. We show that CAP is competitive with prior art and its flexibility unlocks clear benefits for fairness objectives beyond balanced accuracy. Finally, we evaluate CAP on problems with label noise as well as weighted test objectives to showcase how CAP can jointly adapt to different heterogeneities.

==> sec/impact.tex <==
\section{Discussion}\label{sec:con}
We proposed CAP as a flexible method to tackle class heterogeneities and general fairness objectives. CAP achieves high performance by efficiently generating class-specific strategies based on their attributes. We presented strong theoretical and empirical evidence on the benefits of multiple attributes. Evaluations on post-hoc optimization and loss function design revealed that $\name$ substantially improves multiple types of fairness objectives as well as general weighted test objectives. In Appendix D, we also demonstrate the transferability across our strategies: Post-hoc CAP can be plugged in as a loss function to further boost accuracy.

%logit between our two CAP optimization strategies: post-hoc logit adjustment and loss function design, which pave the path for efficiently designing loss function for fairness objectives.

%\section{ and }\label{sec:Lim}
\noindent\textbf{Broader impacts.} Although our approach and applications primarily focus on loss function design and posthoc optimization, CAP approach can also help design class-specific data augmentation, regularization, and optimizers. Additionally, rather than heterogeneities across classes, one can extend CAP-style personalization to problems in multi-task learning and recommendation systems. \textbf{Limitations.} With access to infinite data, one can search for optimal strategies for each class. Thus, the primary limitation of CAP is its multi-task design space that shares the same meta-strategy across classes. However, as experiments demonstrate, in practical finite data settings, CAP achieves better data efficiency, robustness, and test performance compared to individual tuning.

%not the entire design space,In terms of limitations,  tuning all the parameter individually might result in a better strategy. But 

%\xuechen{IN CASE HELPFUL FOR BOARDER IMPACTS: Finally, while we instantiate CAP for the problems of loss function design and posthoc adjustment, CAP-style meta-optimization approaches can have far-reaching consequences to design optimal augmentation, regularization, and optimizers. Overall, this work makes key contributions to fairness and heterogeneous learning problems in terms of methodology as well as practical impact. Personalisation recommendation syatem may reduce the likelihood to experience unexpected and fortuitous items. The probability that people are aware of and use new things will reduce dramatically.}
% \begin{myitemize}

% \item \textbf{Dictionary design:} The attributes and functions should be designed carefully. Adding inappropriate attributes and functions may even hurt the result. As the size of dictionary increases, $\name$ gradually loss benefits.
% \item \textbf{Post-hoc :} $\Delta$ is hard to train in post-hoc so it might influence the transferability from Post-hoc adjustment to Loss Function Design.
% \end{myitemize}
%Personalisation recommendation syatem may reduce the likelihood to experience unexpected and fortuitous items. The probability that people are aware of and use new things will reduce dramatically.

==> sec/intro.tex <==
\section{Introduction}
\begin{figure*}[t]
\vspace{-12pt}
\centering
\begin{tikzpicture}
   \node at (-10.4,0)[anchor=west] {\includegraphics[scale=0.24]{figs/figure_v2.pdf}};
    %\node at (-2.5,1)[anchor=west] [scale=0.5,rotate=-20,opacity=0.7]{Placehoder Figure};
    %\node at (0,0) {\includegraphics[scale=0.5]{./figs/framework.png}};
    
    \def \move {8.5};
    \node at (-10.7+\move,2)[anchor=west] [scale=0.8]{\red{Instantiations of \name:}};
    \node at (-10.4+\move,1.63)[anchor=west] [scale=0.7]{\textbf{1.~Bilevel optimization} of loss function};
    %{\CheckedBox Loss function design via bilevel optimization};
    \node at (-10.4+\move,1.3)[anchor=west] [scale=0.7]{\textbf{2.~Post-hoc optimization} of logits};
    %\node at (-10+\move,1.1)[anchor=west] [scale=0.7]{$\bullet$ Post-hoc logit adjustment $\to$ loss design.};
    %\node at (-10+\move,0.8)[anchor=west] [scale=0.7]{$\bullet$ Bilevel optimization.};
    
    \node at (-10.7+\move,-0.7)[anchor=west] [scale=0.8]{\red{Distinct Heterogeneities (Sec \ref{sec:objective}):}};%y $\to$ Attributes
    \node at (-10.4+\move,-1)[anchor=west] [scale=0.7]{Class frequency};
    %ability $\to$ $\att_{\text{diff}}$ };
    \node at (-10.4+\move,-1.3)[anchor=west] [scale=0.7]{Prediction difficulty};
    %$\to$ $\att_{\text{freq}}$ \& $\att_{\text{norm}}$ };
    \node at (-10.4+\move,-1.6)[anchor=west] [scale=0.7]{Variable class importance};%Distribution shift};
    %$\to$ $\att_{\text{weights}}$};
    \node at (-10.4+\move,-1.9)[anchor=west] [scale=0.7]{Label noise level}; %$\to$$\att_{\text{noise}}$};
    %\node at (-10.4,0.5)[anchor=west] [scale=0.7]{\CheckedBox ...};
    
    
    \node at (-10.7+\move,0.9)[anchor=west] [scale=0.8]{\red{Distinct Fairness Objectives (Sec \ref{sec:attribute}):}};
    \node at (-10.4+\move,0.6)[anchor=west] [scale=0.7]{Balanced error};
    \node at (-10.4+\move,0.3)[anchor=west] [scale=0.7]{Quantiles or Conditional value at Risk};
    \node at (-10.4+\move,0.0)[anchor=west] [scale=0.7]{Standard deviation of class-conditional errors};
    \node at (-10.4+\move,-0.3)[anchor=west] [scale=0.7]{Weighted error};
    %%\node at (-10.4,-2.7)[anchor=west] [scale=0.7]{\CheckedBox ...};
    
    
\end{tikzpicture}
\vspace{-10pt}
\caption{\small{\textbf{Left hand side:} \name views the global dataset as a composition of heterogeneous sub-datasets induced by classes. We extract high-level attributes from these classes and use these attributes to generate class-specific optimization strategies (which correspond to hyperparameters). Our proposal is efficiently generating these hyperparameters based on class-attributes through a meta-strategy. \textbf{Right hand side:} We demonstrate that \name leads to state-of-the-art strategies for loss function design and post-hoc optimization. \name can leverage multiple attributes to flexibly optimize a variety of test objectives under heterogeneities.} }
\end{figure*}\label{fig:framework22}
%Large datasets are a core component of modern deep learning's success. These datasets are often carefully collected and annotated with high-quality labels; the pre-trained models on these datasets significantly boost performance when fine-tuning to multiple tasks~\cite{mahajan2018exploring}. 

%is particularly powerful when we have high-quality large datasets.
%Deep learning is having immense impact in a range of applications going well beyond natural language processing and computer vision. It is becoming

Contemporary machine learning problems arising in natural language processing and computer vision often involve large number of classes to predict. Collecting high-quality training datasets for all of these classes is not always possible, and realistic datasets~\cite{menon2020long,feldman2020does,hardt2016equality} suffer from class-imbalances, missing or noisy labels (among other application-specific considerations). Optimizing desired accuracy objectives with such heterogeneities poses a significant challenge and motivates the contemporary research on imbalanced classification, fairness, and weak-supervision. Additionally, besides distributional heterogeneities, we might have objective heterogeneity. For instance, the target test accuracy may be a particular weighted combination of individual classes, where important classes are upweighted.

%During training, this leads to the scenarios where under-represented or 

%As a result, some classes may be under-represented and require more careful treatments and adjustments. 
% labelsare usually imbalanced and present a long-tailed distribution


%A plausible approach to 
A plausible approach to address these distributional and objective heterogeneities is designing optimization strategies that are tailored to individual classes. A classical example is assigning individual weights to classes during optimization. The recent proposals on imbalanced classification \cite{li2021autobalance,chawla2002smote} can be viewed as generalization of weighting and can be interpreted as developing unique loss functions for individual classes. More generally, one can use class-specific data augmentation schemes, regularization or even optimizers (e.g.~Adam, SGD, etc) to improve target test objective. While promising, this approach suffers when there are a large number of classes $K$: naively learning class-specific strategies would require $\order{K}$ hyperparameters ($\order{1}$ strategy hyperparameter per class). This not only creates computational bottlenecks but also raises concerns of overfitting for tail classes with small sample size.

%of learning class-specific strategies 
%$(\ell_k)_{k=1}^K$ for each class  In this paper, we propose a meta approach to design such class-specific strategies, with emphasis on problems with label-imbalance.

%one can optimize an objective of the form $\Lc(f)=\sum_{k=1}^K \Lc_k(f)$ where $\Lc_k$ is the training loss over the $k$th class and uses a loss function $\ell$


%For instance, frequency or label-noise level are concrete examples of class attributes.
%These class attributes summarize high-level class features such as noise level, imbalance, relative importance, and more. 
To overcome such bottlenecks, we introduce the  \textbf{Class-attribute Priors (\name)} approach. Rather than treating hyperparameters as free variables, \name is a meta-approach that treats them as a function of the class attributes. As we discuss later, example attributes $\att$ of a class include its frequency, label-noise level, training difficulty, similarity to other classes, test-time importance, and more. Our primary goal with \name is building an \textbf{attribute-to-hyperparameter} function $\Strat$ that generates class-specific hyperparameters based on the attributes associated with that class. This process infuses high-level information about the dataset to accelerate the design of class-specific strategies. The $\Strat$ maps the attributes $\att$ to a class-specific strategy $\strat$. The primary advantage is robustness and sample efficiency of $\Strat$, as it requires $\order{1}$ hyperparameters to generate $\order{K}$ strategies. The main contribution of this work is proposing \name framework and instantiating it for loss function design and post-hoc optimization which reveals its empirical benefits. Specifically, we make the following contributions:
\begin{enumerate}
\item \textbf{Introducing Class-attribute Priors (Sec \ref{sec:cap}).} We first provide theoretical evidence on the benefits of using multiple attributes (see Fig \ref{fig:gmmm}). This motivates \name: A meta approach that utilizes the high-level attributes of individual classes to personalize the optimization process. Importantly, \name is particularly favorable to tail classes which contain too few examples to optimize individually.
%Notably, our approach is particularly favorable to tail classes
\item \textbf{\name improves existing approaches (Sec \ref{sec:Exp}).} By integrating \name within existing label-imbalanced training methods, \name not only improves their performance but also increases their stability, notably, AutoBalance \cite{li2021autobalance} and logit-adjustment loss \cite{menon2020long}. 
\item \textbf{\name adapts to fairness objective (Sec \ref{sec:objective}).} \name's flexibility is particularly powerful for non-standard settings that prior works do not account for: \name achieves significant improvement when optimizing fairness objectives other than balanced accuracy, such as standard deviation, quantile errors, or Conditional Value at Risk (CVaR).
\item \textbf{\name adapts to class heterogeneities (Sec \ref{sec:attribute}).} \name can also effortlessly combine multiple attributes (such as frequency, noise, class importance) to boost accuracy by adapting to problem heterogeneity. 
\end{enumerate}

% \item We show the benefit of \name for designing class-specific loss functions, as well as post-hoc logit adjustment, with an emphasis on label-imbalanced problems. Experiments on long-tailed benchmarks reveal that \name strikes a good balance between sample-efficiency and expressivity, and leads to improvements over competing methods, notably, AutoBalance \cite{li2021autobalance} and logit-adjustment loss \cite{menon2020long}. 

% \item  Similarly, \name can effortlessly combine multiple attributes (such as frequency, noise, class importance) to boost accuracy by adapting to problem heterogeneity.
% \end{enumerate}

Finally, while we instantiate \name for the problems of loss-function design and post-hoc optimization, \name can be applied for the design of class-specific augmentations, regularization schemes, and optimizers. This work makes key contributions to fairness and heterogeneous learning problems in terms of methodology, as well as practical impact. An overview of our approach is shown in Fig.~\ref{fig:framework22}
%on heterogeneous problems.
%We show that incorporating multiple class-attributes boost the performance. For instance, jointly using class frequency or 

%While recent imbalanced classification literature placed significant

%The attribute-based prior information boosts performance and is also effective for a noisy dataset.
%\item \textbf{We introduce \dictionary strategy.} We design a \dictionary to implement our API strategy $\Strat$, the experiments demonstrate the benefits of the \dictionary design on CIFAR-LT datasets. It also stabilizes the brittle bi-level algorithm mentioned in \cite{li2021autobalance} by narrowing down the search space.

%\item Our experiments shed light on \textbf{designing loss function in a post-hoc manner}. We exhibit that the post-hoc method can search for loss function at minimum cost, and the desired loss function can be transferred to regular training efficiently.


% where $\strat_y$ is the corresponding adjustment to label $y$. For example, for long-tailed problem, $\strat_y$ is a vector contains $\lb_y, \Deltab_y$ for the aforementioned loss. Furthermore, we notice that the search of $\Strat$ can be done post-hoc and be applied to retrain the model with minimal additional effort. 

%An intuitive approach for loss function design is using a parametric family that enables fine-grained control over individual classes. A good example, that we will focus, is the parametric cross-entropy loss $\ell(y, f(\x))=w_y\log \left(1+\sum_{k \neq y} e^{\lb_{k}-\lb_{y}} \cdot e^{\Deltab_{k} f_{k}(\x)-\Deltab_{y} f_{y}(\x)}\right)$ \cite{menon2020long,ye2020identifying,kini2021label}. This loss contains $O(K)$ hyperparameters (induced by $(w_i\Deltab_i,\lb_i)_{i=1}^K$) where $K$ is the number of classes, leading to a high-dimensional hyperparameter optimization problem.
%Our goal is to obtain a data attribute-based design-function $\Strat$ which
% \usetikzlibrary{math}
% \tikzmath{\move = 1}
% \begin{figure*}[t]
% \vspace{-20pt}
% \centering
% \begin{tikzpicture}
%    \node at (-10.4,0)[anchor=west] {\includegraphics[scale=0.24]{figs/figure_v2.pdf}};
%     %\node at (-2.5,1)[anchor=west] [scale=0.5,rotate=-20,opacity=0.7]{Placehoder Figure};
%     %\node at (0,0) {\includegraphics[scale=0.5]{./figs/framework.png}};
    
%     \def \move {8.5};
%     \node at (-10.7+\move,2)[anchor=west] [scale=0.8]{\red{Instantiations of \name:}};
%     \node at (-10.4+\move,1.63)[anchor=west] [scale=0.7]{\textbf{1.~Bilevel optimization} of loss function};
%     %{\CheckedBox Loss function design via bilevel optimization};
%     \node at (-10.4+\move,1.3)[anchor=west] [scale=0.7]{\textbf{2.~Post-hoc optimization} of logits};
%     %\node at (-10+\move,1.1)[anchor=west] [scale=0.7]{$\bullet$ Post-hoc logit adjustment $\to$ loss design.};
%     %\node at (-10+\move,0.8)[anchor=west] [scale=0.7]{$\bullet$ Bilevel optimization.};
    
%     \node at (-10.7+\move,-0.7)[anchor=west] [scale=0.8]{\red{Distinct Heterogeneities (Sec \ref{sec:objective}):}};%y $\to$ Attributes
%     \node at (-10.4+\move,-1)[anchor=west] [scale=0.7]{Class frequency};
%     %ability $\to$ $\att_{\text{diff}}$ };
%     \node at (-10.4+\move,-1.3)[anchor=west] [scale=0.7]{Prediction difficulty};
%     %$\to$ $\att_{\text{freq}}$ \& $\att_{\text{norm}}$ };
%     \node at (-10.4+\move,-1.6)[anchor=west] [scale=0.7]{Variable class importance};%Distribution shift};
%     %$\to$ $\att_{\text{weights}}$};
%     \node at (-10.4+\move,-1.9)[anchor=west] [scale=0.7]{Label noise level}; %$\to$$\att_{\text{noise}}$};
%     %\node at (-10.4,0.5)[anchor=west] [scale=0.7]{\CheckedBox ...};
    
    
%     \node at (-10.7+\move,0.9)[anchor=west] [scale=0.8]{\red{Distinct Fairness Objectives (Sec \ref{sec:attribute}):}};
%     \node at (-10.4+\move,0.6)[anchor=west] [scale=0.7]{Balanced error};
%     \node at (-10.4+\move,0.3)[anchor=west] [scale=0.7]{Quantiles or Conditional value at Risk};
%     \node at (-10.4+\move,0.0)[anchor=west] [scale=0.7]{Standard deviation of class-conditional errors};
%     \node at (-10.4+\move,-0.3)[anchor=west] [scale=0.7]{Weighted error};
%     %%\node at (-10.4,-2.7)[anchor=west] [scale=0.7]{\CheckedBox ...};
    
    
% \end{tikzpicture}
% \vspace{-15pt}
% \caption{\small{\textbf{Left hand side:} \name views the global dataset as a composition of heterogeneous sub-datasets induced by classes. We extract high-level attributes from these classes and use these attributes to generate class-specific optimization strategies (which correspond to hyperparameters). Our proposal is efficiently generating these hyperparameters based on class-attributes through a meta-strategy. \textbf{Right hand side:} We demonstrate that \name leads to state-of-the-art strategies for loss function design and post-hoc optimization. \name can leverage multiple attributes to flexibly optimize a variety of test objectives under heterogeneities.} }
% \end{figure*}\label{fig:framework22}

\subsection{Related Work}
The existing literature establishes a series of algorithms, including sample weighting~\cite{alshammari2022long,maldonado2022fw,kubat1997addressing,wallace2011class,chawla2002smote}, post-hoc tuning~\cite{menon2020long,zhang2019balance,kim2020adjusting,kang2019decoupling,ye2020identifying}, and loss functions tuning~\cite{cao2019learning,kini2021label,menon2020long,khan2017cost,cui2019class,li2022targeted,tan2020equalization,zhang2017range}, and more \cite{zhang2023deep}. This work aims to establish a principled approach for designing a loss function for imbalanced datasets. Traditionally, a Bayes-consistent loss function such as weighted cross-entropy ~\cite{xie2018snas,morik1999combining} has been used. However, recent work shows it only adds marginal benefit to the over-parameterized model due to overfitting during training. \cite{menon2020long,ye2020identifying,kini2021label} propose a family of loss functions formulated as $\ell(y, f(\x))=\log \left(1+\sum_{k \neq y} e^{\lb_{k}-\lb_{y}} \cdot e^{\Deltab_{k} f_{k}(\x)-\Deltab_{y} f_{y}(\x)}\right)$ with theoretical insights, where $f(\x)$ denotes the output logits of $\x$ and $f_{y}(\x)$ represents the entry that corresponds to label $y$. Above methods determine the value of $\lb$ and $\Deltab$ to re-weight the loss function so the optimization generates a class-balanced model. In addition to these methods, \cite{li2021autobalance} proposes a bilevel training scheme that directly optimizes $\lb$ and $\Deltab$ on a sufficient small imbalanced validation data without the prior theoretical insights. However, the theory-based methods require expertise and trial and error to tune one temperature variable, making it time-consuming and challenging to achieve a fine-grained loss function that carefully handles each class individually. Although the bilevel-based method consider each class separately and personalizes the weight using validation data, optimizing the bilevel problem is typically time-consuming due to the Hessian computations. Bilevel optimization is also brittle, especially when \cite{li2021autobalance} optimizes the inner loss function, which continually changes the inner optima during the training.\\
Regarding the broader goal of fairness with respect to protected groups, the literature contains several proposals  \cite{sahu2018convergence,kleinberg2016inherent}. Balanced error and standard deviation \cite{calmon2017optimized,alabi2018unleashing} between subgroup predictions are widely used metrics. However, they may be insensitive to certain types of imbalances. The Difference of Equal Opportunity (DEO) \cite{kini2021label,hardt2016equality} was proposed to measure true positive rates across groups. \cite{zafar2017fairness} focus on disparate mistreatment in both false positive rate and false negative rate. 
Many modern ML tasks necessitate models with good tail performance, focusing on underrepresented groups. Recent works have introduced techniques that promote better tail accuracy \cite{hashimoto2018fairness,sagawa2019distributionally,sagawa2020investigation,li2021autobalance,kini2020analytic}. The worst-case subgroup error is commonly used in recent papers \cite{kini2021label,sagawa2019distributionally,sagawa2020investigation}. Another popular metric to evaluate the model’s tail performance is the CVaR (Conditional Value at Risk) \cite{williamson2019fairness,zhai2021boosted,michel2021modeling}, which computes the average error over the tails.  Previous works \cite{hashimoto2018fairness,duchi2021learning,hu2018does,michel2021modeling,lahoti2020fairness} also measure tail behaviour using Distributionally Robust Optimization (DRO).


% \subsection{Contributions}
% \textbf{We introduce dictionary strategy.} Motivated by the challenge of original Autobalane algorithm, we proposed dictionary strategy that narrow down the search space. We demonstrate the benefits of the strategy on Cifar10-LT experiments.
% \textbf{We analyze the role of attributes.} We compare the attributes on Cifar10-LT dataset by adding noisy label. 
% \textbf{Post-hoc} We do post-hoc correction and compare multiplicative and additive hyperparameters. We propose that post-hoc could be a simple and efficient way to do loss search.




%  In previous papers \cite{kini2021label}, authors proposed VS loss combining multiplicative weights from CDT loss and additive hyperparameters from LA loss and achieve a good result. A parametric loss function controlled by vectors $\boldsymbol{w}, \boldsymbol{l}, \boldsymbol{\Delta} \in \mathbb{R}^{K}$  was build as $\ell(y, f(\boldsymbol{x}))=w_{y} \log \left(1+\sum_{k \neq y} e^{l_{k}-l_{y}} \cdot e^{\Delta_{k} f_{k}(\boldsymbol{x})-\Delta_{y} f_{y}(\boldsymbol{x})}\right)$. In paper\cite{menon2020long} LA loss use $\iota_{y}=\tau \log \left(N_{y} / N_{\mathrm{tot}}\right)$ and in paper \cite{ye2020identifying} CDT loss use $\Delta_{y}=\left(N_{y} / N_{\max }\right)^{\gamma}$. For those methods, they only tune 1 value ($\tau$ or $\gamma$) and compute the multiplicative or additive weights for each class using class frequency. There are also some shortcomes for those methods, the hyperparameter is tuned by doing grid search which is cursory and inefficient.\\
%  \textbf{Autobalance}
%  A bi-level optimization framework was proposed to design a training loss function which could optimize a blend of accuracy and fairness-seeking objectives in \cite{li2021autobalance}. It could jointly training the model and the loss function hyperparameters. The parametric loss function is same as the VS-loss introduced in \cite{kini2021label}.\\
%  But there are still some challenges. The bi-level optimization face the stability problem. During the training, there are some sudden step of the hyperparameter. There are strict restrictions for warm-up and learning rate. In bilevel training, the warm-up phase is essential to guarantee that the IFT assumption \cite{lorraine2020optimizing} $\frac{\partial \mathcal{L}_{\text {train }}\left(\boldsymbol{\theta}^{\star}, \boldsymbol{\alpha}^{\star}\right)}{\partial \boldsymbol{\theta}}=0$ is approximately satisfied. The difficulty of hypergradient estimation also influence the training.


==> sec/main.tex <==
%!TEX root = ../automl.tex
\section{Experiments and Main Results}\label{sec:Exp}
% \input{sec/tab_bilevel}
\input{./sec/obj_img}
\begin{table*}
\begin{center}\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
%\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
%\toprule
\multicolumn{1}{l}{Post-hoc methods}                  & $\berr$              & $\dev$ & $\cva{0.2}$ &$\quana{0.2}$ &$\werr$ \\
\midrule
$\pretrain$&        61.94 ($\pm$0.28)        & 27.13($\pm$0.35)  & 96.95($\pm$0.15)  &  93.01($\pm$0.58) &62.53($\pm$0.53) \\
  $\nodic_{\text{Post-hoc}}$     &    -1.62($\pm$0.36)            & -8.51($\pm$0.75)   & -11.48($\pm$0.81)  & -12.79($\pm$0.43) &-2.82($\pm$0.56)  \\
  $\text{LA}_{\text{Post-hoc}}$  &       -3.73($\pm$0.29)        & -8.72($\pm$0.66)   & -12.21($\pm$0.50)  & -15.01($\pm$0.35) &  -3.62($\pm$0.37) \\
 % $\name_{\text{Post-hoc}}$: Single attribute     &    -4.30($\pm$0.26)           & \textbf{-13.99}($\pm$0.21)   & -14.28($\pm$0.92)  & -17.68($\pm$0.12) & -4.03($\pm$0.52)  \\
 % %$\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
 % $\name_{\text{Post-hoc}}$: Combined attributes &  \textbf{-4.36}($\pm$0.25)   &  \textbf{-13.92}($\pm$0.24)  & \textbf{-14.75}($\pm$0.87)  & \textbf{-18.34}($\pm$0.47) & \textbf{-6.21}($\pm$0.49)\\
 $\name_{\text{Post-hoc}}$ &  \textbf{-4.36}($\pm$0.25)   &  \textbf{-13.92}($\pm$0.24)  & \textbf{-14.75}($\pm$0.87)  & \textbf{-18.34}($\pm$0.47) & \textbf{-6.21}($\pm$0.49)\\
\bottomrule
		\end{tabular}}\vspace{-5pt}\caption{The error difference between other approaches compared to pre-trained model. The first line shows the performance of Pretrained model, and the following line shows the error difference of other methods (smaller is better). For objectives with $a$, we set $a = 0.2$. This is commonly used for difficult or few classes in other papers\cite{zhai2021boosted,liu2019large}. 
		%Then the target classes of quantile classes errors and conditional value of errors is the 20th and 0th-20th worst classes. 
		%For $\dev$, which quantifies the similarly for class-conditional errors, $\quan$ and $\cv$ ,which focus on tail behavior, $\att_{\text{diff}}$ could achieve better result. For weighted test error \eqref{weighted obj}, incorporating weights into CAP leads to significant improvement (results averaged over multiple random weights).
		}\label{table:attributes_objective}
	\end{center}
\end{table*}
In this section, we present our experiments in the following way. Firstly, we demonstrate the performance of $\name$ on both loss function design via bilevel optimization and post-hoc logit adjustment in Sec.~\ref{sec:bilevel}. 
%We further highlight the connection between bilevel $\name$ and post-hoc optimization by transferring the learned hyper-parameters.
Sec.~\ref{sec:objective} demonstrates that \name provides noticeable improvements for fairness objectives beyond balanced accuracy. Then Sec.~\ref{sec:attribute} discusses the advantage of utilizing attribute\red{s} and how $\name$ leverages them in noisy, long-tailed datasets through perturbation experiments. Lastly, we defer the experiment details including hyper-parameters, number of trails, and other reproducibility information to appendix.

\noindent\textbf{Dataset.} In line with previous research \cite{menon2020long,ye2020identifying,li2021autobalance}, we conduct the experiments on CIFAR-LT and ImageNet-LT datasets. The CIFAR-LT modifies the original CIFAR10 or CIFAR100 by reducing the number of samples in tail classes. The imbalance factor, represented as $\rho = N_{max} / N_{min}$, is determined by the number of samples in the largest ($N_{max}$) and smallest ($N_{min}$) classes. To create a dataset with the imbalance factor, the sample size decreases exponentially from the first to the last class. We use $\rho=100$ in all experiments, consistent with previous literature. The ImageNet-LT, a long-tail version of ImageNet, has 1000 classes with an imbalanced ratio of $\rho=256$. The maximum and minimum samples per class are 1280 and 5, respectively. During the search phase for bilevel $\name$,
%and post-hoc transferability experiments (Sec.~\ref{sec:bilevel}),
we split the training set into 80\% training and 20\% validation to obtain the optimal loss function design. We remark that the validation set is imbalanced, with tail classes containing very few samples, making it challenging to find optimal hyper-parameters without overfitting. For all other post-hoc experiments (Sec.~\ref{sec:objective} and \ref{sec:attribute}), we follow the setup of \cite{menon2020long,hardt2016equality} by training a model on entire training dataset as the pre-train model, and optimizing a logit adjustment $g$ on a balanced validation dataset. Additionally, all CIFAR-LT experiments use ResNet-32 \cite{he2016deep}, and ImageNet-LT experiments use ResNet-50.
%, in accordance with literature.

\subsection{$\name$ Improves Prior Methods Using Post-hoc or Bilevel Optimization} \label{sec:bilevel}

This section presents our loss function design experiments on imbalanced datasets by incorporating  \name into the training scheme of \cite{li2021autobalance,menon2020long, ye2020identifying}, as discussed in Sec.~\ref{sec:imp_bilevel_posthoc}. Table~\ref{table:dic} demonstrates our results.  The first part displays the outcomes of various existing methods with their optimal hyper-parameters.  It is worth noting that the original best results for single-level methods (\cite{menon2020long, ye2020identifying}) are obtained from grid search on the test dataset, which leads to much better performance than our reproduced results using validation grid search in Table.~\ref{table:dic}. Moreover, both of the grid search methods demand substantial computation budgets. As illustrated in the second part of Table~\ref{table:dic}, bilevel and post-hoc $\name$ significantly improve the balanced error across all datasets. %We also conduct experiments to further bridge the connection between post-hoc and bilevel loss function design, as discussed in Sec.\ref{sec:attributes}, which can be found in Appendix~\ref{app:transfer}.

%\noindent\textbf{Transferability from post-hoc optimization to loss function design.} In parametric cross entropy loss $\ell(y, f(\x))=\log \left(1+\sum_{k \neq y} e^{\Deltab_{k} f_{k}(\x)+\lb_{k}-\Deltab_{y} f_{y}(\x)-\lb_{y}}\right)$, the output logits are adjusted by $\Deltab f(\x)-\lb$ which paves the path of searching a post-hoc $\Strat'$ and transfer to \name $\Strat$. \cite{menon2020long} provides the post-hoc optimization $\lb'$ by flipping the sign of $\lb$ in loss adjustment. In our approach, we search a post-hoc $\Strat'$ with very marginal computation cost to obtain post-hoc $\lb'$ and $\Deltab'$, the training loss function can be transferred from post-hoc as $\ell(y, f(\x))=\log \left(1+\sum_{k \neq y} e^{{\Deltab'}_{k}^{-1} f_{k}(\x)-{\lb'}_{k}-{\Deltab'}_{y}^{-1} f_{y}(\x)+{\lb'}_{y}}\right)$.

%Additionally, we implement the $\name$ version of LA by searching the weight $\tau$ for LA loss. As we discussed in Sec.~\ref{sec:attributes}, $\name$ can generalize to LA by selecting frequency as the only attribute and tuning a single entry of $\w_\lb$. We also conduct experiments to further bridge the connection between post-hoc and bilevel loss function design, as discussed in Sec.\ref{sec:attributes}, which can be found in Appendix~\ref{app:transfer}.

% This section presents our loss function design experiments on imbalanced datasets, adopting the training process and configuration from \cite{li2021autobalance}  which splits the train dataset into 80\% training and 20\% validation. We utilize class frequency $\attfreq$ as the sole attribute. For function $\bm{\Func}$, we employ both logarithm and polynomial functions. In total, we optimize 6 parameters, significantly reducing the search space compared to \cite{li2021autobalance}, which varies from 20 to 100 parameters. The results are shown in Table~\ref{table:dic}. The first part displays the outcomes of various existing methods with their optimal hyper-parameters. We note that the hyper-parameters for single-level methods (\cite{menon2020long, ye2020identifying}) are obtained from grid search, demanding substantial computation budgets. As illustrated in the second part of Table~\ref{table:dic}, bilevel $\name$ significantly improves the balanced error across all datasets. Moreover, we implement the $\name$ version of LA by searching the weight $\tau$ for LA loss. As we discussed in Sec.~\ref{sec:attributes}, $\name$ can generalize to LA by selecting frequency as the only attribute and tuning a single entry of $\w_\lb$. 
% The results indicate that incorporating additional functions $\Fc$ further enhances performance, and several dictionary entries are necessary to achieve fine-grained control over loss function design.

%  A special version of $\name$ is tunning $\tau$ for LA loss and $\gamma$ for CDT loss. This is actually same as $\name$ with only 1 row dictionary $\boldsymbol{D} \in \mathbb{R}^{1 \times K}$. The result shows one function is not enough, and we need a dictionary that can control the freedom of training. Finally, We show the result of our method $\name_{AB}$. It can design a better loss function and outperform other benchmarks. In Figure\ref{fig:stable}, the value of the hyperparameters changes dramatically, and even the sort of the hyperparameters for each class changes. After adding the dictionary strategy, the training is much more stable. Also, $\name$ makes it possible to do bilevel optimization without warm-up and get highly competitive results. This also shows that $\name$ could solve the instability issue in Autobalance to a large extent. As shown in Table\ref{table:warmup_result}\xuechen{to appendix}, warm-up in a more balanced way could get better results. If the search phase starts with biased model parameters, it's hard to escape and will influence the final result. This could also explain why the without warm-up version could achieve a good result.\xuechen{remove warm-up discussion? in appendix?}

% \begin{table}[t]
% 	\small
% 	\begin{center}\resizebox{0.6\textwidth}{!}{
% 			\begin{tabular}{lccc}
% 			\toprule
% 			& & CIFAR10 & CIFAR100\\
% 				\toprule
% 				{\multirow{3}{*}{Vanilla}}               			                & CE       & 30.45           &  62.69 \\ \cline{2-4}
% 				            & LA       & 20.36            &  57.13 \\ \cline{2-4}
% 			                & CDT      & 20.73      & 57.29\\ 
% 			\midrule
% 			{\multirow{3}{*}{AutoBalance}} & no init    & 21.39 &56.84\\  \cline{2-4}
% 			& LA init    & 21.15 &56.70 \\ 
% 				\midrule
% 			{\multirow{5}{*}{$\name_{\text{AB}}$}} & $\tau$ for LA loss    & 21.82 &58.68\\  \cline{2-4}
% 			& $\gamma$ for CDT loss    & 22.67 &58.41\\  
% 			\cline{2-4}
% 			 & no init    & 20.41 &56.64\\ \cline{2-4}
% 			& LA init    & 20.22 &56.57\\  \cline{2-4}
% 			& without warm up & 20.16 &56.56\\ 
% 				\bottomrule %\vspace{10pt}
% 		\end{tabular}}\caption{Evaluations of balanced accuracy on long-tailed data. LA loss is proposed in paper \cite{menon2020long}, CDT is proposed in paper \cite{ye2020identifying} and AutoBalance is proposed in paper \cite{li2021autobalance}}\label{table:dic}\vspace{-10pt}
% 	\end{center}
% \end{table}
 
% \begin{table}[t]
% 	\small
% 	\begin{center}\resizebox{0.4\textwidth}{!}{
% 			\begin{tabular}{llll}
% 				\toprule
%                               &       & $\err_{\mathrm{bal}}(f)$&$\mathcal{S}(f)$               \\
% \toprule
% \multicolumn{1}{l}{\multirow{3}{*}{$\name_{\text{AB}}$}}   & $\att_{freq}$        & 39.84&0.26 \\\cline{2-4} 
% \multicolumn{1}{l}{}                          & $\att_{diff}$       & 40.78&0.14  \\\cline{2-4} 
% \multicolumn{1}{l}{}                          & $\att_{freq}$ \& $\att_{diff}$ & 38.79&0.20  \\ 
% \midrule
% \multicolumn{2}{l}{AutoBalance}                             & 40.04&0.31  \\ 
% \bottomrule
% 		\end{tabular}}\caption{Evaluations on long-tailed data with noisy label.}\label{table:attributes}\vspace{-5pt}
% 	\end{center}
% \end{table}

% \begin{table}[t]
% 	\begin{minipage}{.5\linewidth}
% 		%\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 		 	\begin{tabular}{lccc}
% 			\toprule
% 			& & CIFAR10 & CIFAR100\\
% 				\toprule
% 				{\multirow{3}{*}{Vanilla}}               			                & CE       & 30.45           &  62.69 \\ \cline{2-4}
% 				            & LA       & 20.36            &  57.13 \\ \cline{2-4}
% 			                & CDT      & 20.73      & 57.29\\ 
% 			\midrule
% 			{\multirow{3}{*}{AutoBalance}} & no init    & 21.39 &56.84\\  \cline{2-4}
% 			& LA init    & 21.15 &56.70 \\ 
% 				\midrule
% 			{\multirow{5}{*}{$\name_{\text{AB}}$}} & $\tau$ for LA loss    & 21.82 &58.68\\  \cline{2-4}
% 			& $\gamma$ for CDT loss    & 22.67 &58.41\\  
% 			\cline{2-4}
% 			 & no init    & 20.41 &56.64\\ \cline{2-4}
% 			& LA init    & 20.22 &56.57\\  \cline{2-4}
% 			& without warm up & 20.16 &56.56\\ 
% 				\bottomrule %\vspace{10pt}
% 		\end{tabular}}\caption{Evaluations of balanced accuracy on long-tailed data. LA loss is proposed in paper \cite{menon2020long}, CDT is proposed in paper \cite{ye2020identifying} and AutoBalance is proposed in paper \cite{li2021autobalance}}\label{table:dic}\vspace{-10pt}
% 	\end{center}
% 		%\end{table}
% 	\end{minipage}\hspace{10pt}\begin{minipage}{.52\linewidth}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{llllll}
% 			\toprule
% 			\multicolumn{2}{l}{}              & \multicolumn{2}{l}{CIFAR10}& \multicolumn{2}{l}{CIFAR100} \\
% 				\toprule
% 				\multicolumn{2}{l}{}              & search phase & retrain& search phase & retrain \\ 
% 		\toprule		
% \multicolumn{1}{l}{\multirow{2}{*}{\xuechen{unfair:}Vanilla}}   & $\tau$ for LA  & 20.93        & 21.35&58.14&57.13   \\\cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\gamma$ for CDT                 & 23.48        & 21.73 &58.51&57.26  \\ 
% \midrule
%     \multicolumn{1}{l}{\multirow{3}{*}{Post-hoc}}   & $\boldsymbol{l}$                      & 20.90        & 21.71 &57.98&57.82  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{\Delta}$                      & 23.74        & 24.06 &58.61&58.80  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{l}$\&$\boldsymbol{\Delta}$                  & 23.41        & 23.38 &57.80&58.57  \\                  

% \midrule

% \multicolumn{1}{l}{\multirow{3}{*}{$\name_{\text{Post-hoc}}$}}   & $\boldsymbol{l}$                      & 20.76        & 20.48 &57.67&57.06  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{\Delta}$                      & 22.64        & 20.93  &58.49&57.09 \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{l}$\&$\boldsymbol{\Delta}$                  & 21.66        & 21.05 &57.68&57.23  \\ 
% \bottomrule
% 		\end{tabular}}\caption{Evaluations on long-tailed data.}\label{table:posthoc}\vspace{-5pt}
% 	\end{center}
% 	\end{minipage}\vspace{-5pt}
% \end{table}

%\input{./sec/tab_posthoc}
%\subsection{Connection to post-hoc adjustment}\label{sec:posthoc}

% \noindent{\textbf{Connection to post-hoc adjustment}}\label{sec:posthoc} To better understand the potential of $\name$ and the connection between loss function design and post-hoc adjustment, we design an experiment with results shown in Table~\ref{table:posthoc}. In this experiment, we use the same \dictionary, split the original training data to $80\%$ train and $20\%$ validation, and train a model $f$ using regular cross-entropy loss on the $80\%$ train set as the pre-trained model, which is biased toward the imbalanced distribution. Our goal is to find a post-hoc adjustment $g$ so that $g\circ f$ achieves minimum balanced loss on the $20\%$ validation set. In Table~\ref{table:posthoc}, the searching phase displays the test error of adjusted model $g\circ f$. Following the transferability discussion in Sec.~\ref{sec:imp_bilevel_posthoc}, we use the searched post-hoc adjustment as the loss function design to retrain the model from scratch on the entire training dataset. Interestingly, retraining further improves the post-hoc performance. As post-hoc adjustment requires only about 1/5 of the time and fewer computational resources than loss function design, it provides a simple and efficient approach for loss function design. We also observe that training $\w_\lb$ along with $\w_\Deltab$ leads to performance degradation compared to only training $\w_\lb$, and training only $\w_\Deltab$ also performs worse than $\w_\lb$. In supplementary materials \ref{app:transfer}, we conduct more experiments and provide explanations for this phenomenon.

% \xuechen{
% \noindent{\textbf{Connection to post-hoc adjustment}}\label{sec:posthoc} To better understand the potential of $\name$ and the connection between loss function design and post-hoc adjustment, we conduct more experiments and provide explanations, shown in supplementary materials \ref{app:transfer}.}

% We first train the whole model $f: \mathcal{X} \rightarrow \mathbb{R}^{K}$ using the whole long-tailed training dataset. As we are using simple cross entropy, the result is biased with balanced error $\err_{\mathrm{bal}}(f)$ 30.45. We use a small subset of test dataset as validation dataset to train the post-hoc $g_{\boldsymbol{\alpha}}$ contains parameters $\boldsymbol{\alpha}=\left(l_{y}, \Delta_{y}\right)_{y=1}^{K}$. So post-hoc is $g_{\boldsymbol{\alpha}} \circ f\left(\boldsymbol{x}\right) = \frac{f_{y}\left(\boldsymbol{x}\right)}{\sigma\left(\Delta_{y}\right)}-l_{y}$ For CIFAR10, if we have more than 50 samples in each class, the post-hoc model could be well trained. The input of post-hoc $g_{\boldsymbol{\alpha}} $ is only the logits value $f(x) \in \mathbb{R}^{K}$. 
% $\hat{g}=\arg \min _{\boldsymbol{\alpha} \in \mathcal{A}} \frac{1}{K} \sum_{i=1}^{K} \mathcal{L}_{k}\left(\boldsymbol{y}, g \circ f\left(\boldsymbol{x}\right)\right)$. After post-hoc correction, we use ${\sigma\left(\Delta_{y}\right)}$ and $l_{y}$ directly to adjust the loss and retrain. We do this experiment to discover is post-hoc could be a way to tune the loss.\\

% \textbf{Results and discussion} 
% The result of post-hoc training was shown in Table\ref{table:posthoc}. Just using post-hoc, which takes only about 1/5 of the time and also much less computing resources compared to autobalance, could get a highly competitive result. Dictionary strategy also works for post-hoc training. More interesting, after using the dictionary strategy, hyperparameters trained with post-hoc could be used to adjust loss directly and get even better performance. So post-hoc could be used as a simple and efficient way to search loss. We also compare $\Delta$ and $l$ for post-hoc. For post-hoc training, using only $l$ could get better results. $\Delta$ is much harder to train. That might be because of adjusting logits using additive weights is the same as moving the boundary directly, while the influence of multiplicative weights is much more complex. But $\Delta$ works well in the retraining phase. 

% By adding attributes which is correlated to difficulty, we could improve the worse case accuracy without hurting balanced accuracy. This always happen at the end of the training. The result for balanced CIFAR10 also verify this conclusion. (balanced acc: 92.9 to 93.06, worst class accuracy: 83.4 to 85.5)

% \multicolumn{1}{l}{\multirow{3}{*}{Post-hoc with dictionary: Imbalanced Val(10 samples for minority class)}} & ly                      & 22.84        & 22.63   \\ \cline{2-4} 
% \multicolumn{1}{l}{}                                         & $\Delta$                      & 24.43        & 24.35   \\ \cline{2-4} 
% \multicolumn{1}{l}{}                                         & ly\&$\Delta$                  & 22.97        & 22.78   \\ 
% \midrule




% \begin{table}[t]
% 	\small
% 	\begin{center}\resizebox{0.8\textwidth}{!}{
% 			\begin{tabular}{llllll}
% 			\toprule
% 			\multicolumn{2}{l}{}              & \multicolumn{2}{l}{CIFAR10}& \multicolumn{2}{l}{CIFAR100} \\
% 				\toprule
% 				\multicolumn{2}{l}{}              & search phase & retrain& search phase & retrain \\ 
% 		\toprule		
% \multicolumn{1}{l}{\multirow{2}{*}{Vanilla}}   & $\tau$ for LA  & 20.93        & 21.35&58.14&57.13   \\\cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\gamma$ for CDT                 & 23.48        & 21.73 &58.51&57.26  \\ 
% \midrule
%     \multicolumn{1}{l}{\multirow{3}{*}{Post-hoc}}   & $\boldsymbol{l}$                      & 20.90        & 21.71 &57.98&57.82  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{\Delta}$                      & 23.74        & 24.06 &58.61&58.80  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{l}$\&$\boldsymbol{\Delta}$                  & 23.41        & 23.38 &57.80&58.57  \\                  

% \midrule

% \multicolumn{1}{l}{\multirow{3}{*}{$\name_{\text{Post-hoc}}$}}   & $\boldsymbol{l}$                      & 20.76        & 20.48 &57.67&57.06  \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{\Delta}$                      & 22.64        & 20.93  &58.49&57.09 \\ \cline{2-6} 
% \multicolumn{1}{l}{}                                         & $\boldsymbol{l}$\&$\boldsymbol{\Delta}$                  & 21.66        & 21.05 &57.68&57.23  \\ 
% \bottomrule
% 		\end{tabular}}\caption{Evaluations of balanced accuracy on long-tailed data.}\label{table:posthoc}\vspace{-10pt}
% 	\end{center}
% \end{table}

\subsection{Benefits of $\name$  for Optimizing Distinct Fairness Objectives}\label{sec:objective}
\begin{table*}
    \centering
	\resizebox{\textwidth}{!}{
			\begin{tabular}{lllllll}
				\toprule
\multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{2}{l}{CIFAR100-LT} & \multicolumn{2}{l}{ImageNet-LT} & \multicolumn{2}{l}{CIFAR10-LT+Noise}\\
\toprule
\multicolumn{1}{l}{}                  & $\berr$&$\dev$ & $\berr$&$\dev$            & $\berr$&$\dev$          \\
\midrule
Cross entropy &  61.94($\pm$0.28)              &    27.13($\pm$0.35)         &  55.59($\pm$0.26)              &   29.10($\pm$0.64)       &43.76($\pm$0.74) & 31.69($\pm$0.81) \\
 $\nodic_{\text{Bilevel}}$ (AutoBalance \cite{li2021autobalance})     &  56.70($\pm$0.32)              &    20.13($\pm$0.68)         &  50.93($\pm$0.16)              &   26.06($\pm$0.61)      &40.04($\pm$0.79) &   36.30($\pm$0.89)    \\
 $\name_{\text{Bilevel}}$: $\att_{\textsc{freq}}$     &  56.64 ($\pm$0.21)             &    19.10($\pm$0.67)         &  50.82($\pm$0.13)               &   24.36($\pm$0.49)       & 39.91($\pm$0.66)&  26.54($\pm$0.80)    \\
                           $\name_{\text{Bilevel}}$: $\att_{\textsc{diff}}$     &  58.27($\pm$0.24)              &   \textbf{17.62}($\pm$0.65)             &     52.97($\pm$0.30)  &           \textbf{21.28}($\pm$0.58)       & 40.61($\pm$0.61)&  \textbf{14.49}($\pm$0.72)   \\
                           $\name_{\text{Bilevel}}$: $\att_{\textsc{freq}}$+$\att_{\textsc{diff}}$  &   \textbf{56.38}($\pm$0.19)             &     18.53($\pm$0.63)           &    \textbf{49.31}($\pm$0.34)            &  22.14($\pm$0.46)            & \textbf{38.36}($\pm$0.79)&
19.78($\pm$0.75) \\
\bottomrule
		\end{tabular}}\caption{Attributes help optimization adapt to dataset heterogeneity. We conduct experiments using bilevel loss design and report the balanced misclassification error,and standard deviation of class-conditional errors with different class-specific attributes.}\label{table:attributes_lt}\vspace{-10pt}

\end{table*}
% 		\begin{table*}
% 	\begin{center}\resizebox{0.8\textwidth}{!}{
% 			\begin{tabular}{llllll}
% 				\toprule
% %\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
% %\toprule
% \multicolumn{1}{l}{Post-hoc methods}                  & $\berr$              & $\dev$ & $\cva{0.2}$ &$\quana{0.2}$ &$\werr$ \\
% \midrule
% $\pretrain$&        61.94 ($\pm$0.28)        & 27.13($\pm$0.35)  & 96.95($\pm$0.15)  &  93.01($\pm$0.58) &62.53($\pm$0.53) \\
%   $\nodic_{\text{Post-hoc}}$     &    -1.62($\pm$0.36)            & -8.51($\pm$0.75)   & -11.48($\pm$0.81)  & -12.79($\pm$0.43) &-2.82($\pm$0.56)  \\
%   $\text{LA}_{\text{Post-hoc}}$  &       -3.73($\pm$0.29)        & -8.72($\pm$0.66)   & -12.21($\pm$0.50)  & -15.01($\pm$0.35) &  -3.62($\pm$0.37) \\
%  % $\name_{\text{Post-hoc}}$: Single attribute     &    -4.30($\pm$0.26)           & \textbf{-13.99}($\pm$0.21)   & -14.28($\pm$0.92)  & -17.68($\pm$0.12) & -4.03($\pm$0.52)  \\
%  % %$\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
%  % $\name_{\text{Post-hoc}}$: Combined attributes &  \textbf{-4.36}($\pm$0.25)   &  \textbf{-13.92}($\pm$0.24)  & \textbf{-14.75}($\pm$0.87)  & \textbf{-18.34}($\pm$0.47) & \textbf{-6.21}($\pm$0.49)\\
%  $\name_{\text{Post-hoc}}$ &  \textbf{-4.36}($\pm$0.25)   &  \textbf{-13.92}($\pm$0.24)  & \textbf{-14.75}($\pm$0.87)  & \textbf{-18.34}($\pm$0.47) & \textbf{-6.21}($\pm$0.49)\\
% \bottomrule
% 		\end{tabular}}\vspace{-10pt}\caption{The error difference between other approaches compared to pre-trained model. The first line shows the performance of Pretrained model, and the following line shows the error difference of other methods (smaller is better). For objectives with $a$, we set $a = 0.2$. This is commonly used for difficult or few classes in other papers\cite{zhai2021boosted,liu2019large}. 
% 		%Then the target classes of quantile classes errors and conditional value of errors is the 20th and 0th-20th worst classes. 
% 		%For $\dev$, which quantifies the similarly for class-conditional errors, $\quan$ and $\cv$ ,which focus on tail behavior, $\att_{\text{diff}}$ could achieve better result. For weighted test error \eqref{weighted obj}, incorporating weights into CAP leads to significant improvement (results averaged over multiple random weights).
% 		}\label{table:attributes_objective}\vspace{-10pt}
% 	\end{center}
% \end{table*}
Recent works on label-imbalance places a significant emphasis on the balanced accuracy evaluations \cite{menon2020long,li2021autobalance,cao2019learning}. However, in practice, there are many different fairness criteria and balanced accuracy is only one of them. In fact, as we discuss in \eqref{weighted obj}, we might even want to optimize arbitrary weighted test objectives. In this section, we demonstrate the flexibility and merits of $\name$ when optimizing fairness objectives other than balanced accuracy. The experiments are conducted on the CIFAR100-LT dataset using the post-hoc approaches. For the fairness objectives, we mainly focus on three objectives: quantile class error $\quan$, conditional value at risk (CVaR) $\cv$, and the combined risk $\aggr$, which consists of standard deviation of error and the regular classification error. 

We first demonstrate the performance on quantile class error $\quan = \mathbb{P}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]$, where $\mathrm{K}_{a}$ denotes the class index with the worst $\lceil\mathrm{K}\times{a}\rceil$-th error. For instance, in CIFAR100-LT, where $K=100$, $\quana{0.2}$ denotes the test error of the worst 20 percentile class. That is, we sort the classes in descending order of test error and return the error of the class 20\%th class ID. Thus, each selection of $a$ raises a new objective. Fig.~\ref{fig:obj_quan} shows the improvement over the pre-trained model when optimizing $\quan$ with multiple selections of $a$. We observe that $\name$ significantly outperforms both logit adjustment and plain post-hoc. 

$\cv = \mathbb{E}\left[\err_{k}\mid \err_{k}>\quan\right]$ measures the average error of  $\lceil\mathrm{K}\times{a}\rceil$ classes with worst errors. Instead of $\quan$, which only focuses on the specific quantile class error, optimizing the $\cv$ tend to improve the tail behavior of the classifier, which is a more general fairness objective. Fig.~\ref{fig:obj_cv} shows the test improvements over three approaches, and $\name$  is consistently better than all other methods. 

Finally, for the combined risk $\aggr$, we define $\aggr = \lambda\cdot\serr+(1-\lambda)\cdot\dev$ where $\serr$ is the regular classification error and $\dev$ denotes the standard deviation of classification errors. We plot the error-deviation curve by varying $\lambda$ from 0 to 1 with stepsize 0.1 on three approaches in Fig.~\ref{fig:obj_agg}, each point corresponds to a different $\lambda$. We observe that plain post-hoc cannot achieve a small standard deviation, and post-hoc LA degrades when achieving smaller $\dev$, $\name$ accomplish the best performance and are flexible to adapt to different objectives.

When using plain post-hoc (without CAP), each class parameter is updated individually. Thus, optimizing for specific classes (e.g., $\quan$) dramatically hurts the performance of other classes which are ignored. Confirming this, we found that optimizing plain post-hoc is unstable and does not achieve decent results. On the other hand, while post-hoc LA outperforms plain post-hoc, optimizing only one temperature variable lacks fine-grained adaptation to various objectives. In contrast, $\name$ achieves a noticeably better performance on all objectives thanks to its best of both worlds design.
%flexible design space since $\name$ uses class attributes and fine-grained control into consideration.

Table~\ref{table:attributes_objective} shows more results.  $\werr$ denotes a weighted test objective induced by weights $\bm{\omega}^{\text{test}}_k\in\R^K$ given by\vspace{-0pt}
\begin{align}
\vspace{-20pt}
    \werr=\sum_{k=1}^{K}{\bm{\omega}^{\text{test}}_k\err_{k}}\quad\text{where}\quad \sum_{k=1}^K\bm{\omega}^{\text{test}}_k=K.\label{weighted obj}
    \vspace{-20pt}
\end{align} 
%We report the average result of 10 trails of different $\bm{\omega}^{\text{test}}$ for $\werr$. At each trial, weights $\bm{\omega}^{\text{test}}_k$ are generated i.i.d.~from the uniform distribution over $[0,1]$. We consider the three attributes highlighted in Table \ref{table:attributes_definition}, namely $\attfreq,\attdiff,\attw$. For each test objective, we report the single best attribute as well as combination of all attributes. 

% We found that the best attribute for $\berr,\werr$ are $\attfreq$ and for $\dev,\cv,\quan$ are $\attdiff$. Observe that $\attw$ is not informative for unweighted objectives $\berr,\dev,\cva{0.2},\quana{0.2}$, thus these only use $\attfreq$ and $\attdiff$ for the ``All attributes'' row.

Overall, Table~\ref{table:attributes_objective} shows that $\name$ consistently achieves the best results on multiple fairness objectives. An important conclusion is that, the benefit of \name is more significant for objectives beyond balanced accuracy and improvements are around 2\% or more (compared to \cite{menon2020long} or plain post-hoc). This is perhaps natural given that prior works put an outsized emphasis on balanced accuracy in their algorithm design  \cite{menon2020long,li2021autobalance}.

% \xuechen{define objectives here?}
% In this section, all the results are generated via post-hoc adjustment. We mainly discussed the benefits of $\name$ with three different objectives. In setting A and B, we plot the improvement of post-hoc adjustment for objective $\quan = \mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]$($\mathrm{K}_{a}$ are the quantile classes determined by level $\mathrm{a}$) and $\cv = \mathbb{E}\left(\err_{k}\mid \err_{k}>\quan\right)$ at different level $a$. For clarification, the sort of classes is not generated by the original class id or class frequency. It's the sequence number of classes in descending order based on performance. These two objectives both measure the error of target classes. $\quan$ focuses on quantile classes while $\cv$ focuses on tail behavior which is the performance of classes more difficult than quantile classes. In Setting B, post-hoc  adjustment was used to optimize aggregation of two different objectives, standard deviation $\dev$ and standard error $\serr$, $\aggr = \lambda*\serr+(1-\lambda)*\dev$. We plot the two objectives $\dev$ and $\serr$ for various $\lambda$ value. Our $\name$ result is competitive with the most unrestricted method $\nodic$ post-hoc and LA post-hoc with strict restrictions. We also contains $werr$ objective. Instead of balanced accuracy, we evaluate the error on a new class distribution. The target weight is generated uniform randomly. We repeat the experiment ten times with random seeds from 100 to 1000.\\



%  Standard deviation of class-conditional errors $\dev = \text{std}(\err)$,
%  Conditional value of errors at level $\cv = \mathbb{E}\left(\err_{k}\mid \err_{k}>\quan\right)$ and Weighted misclassification error $\werr=(1 / K) \sum_{k=1}^{K}w\err_{\mathrm{k}}$.



% \textbf{Results and discussion}  In Figure\ref{fig:obj_quan} and \ref{fig:obj_cv}, with different $a$ value, our method $\name$ always greater than baseline(LA and Plain post-hoc adjustment). When training to optimize these two objectives, parameters are updated with samples from small changing subsets of classes influenced by current class-conditional errors. Without general prior information, the parameter of each class was updated individually. Improving the accuracy of current target classes may dramatically hurt other classes' performance and change the sort of class errors. The plain post-hoc adjustment is unstable and couldn't achieve good results. La post-hoc training with too strict restrictions couldn't adapt to various objectives and adjust for target classes, so the result is still worse. Figure\ref{fig:obj_agg} shows the result of setting C. Our method $\name$ exhibits a noticeably better tradeoff curve. It could achieve smaller deviation for the same standard error. Table\ref{table:attributes_objective} presents the result for various objectives. Our method always outperforms SOTA methods. 
%\subsection{Implementation details}\label{sec:imp}
% \begin{table*}
%     \centering
% 	\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lllllll}
% 				\toprule
% \multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{2}{l}{CIFAR100-LT} & \multicolumn{2}{l}{ImageNet-LT} & \multicolumn{2}{l}{CIFAR10-LT+Noise}\\
% \toprule
% \multicolumn{1}{l}{}                  & $\berr$&$\dev$ & $\berr$&$\dev$            & $\berr$&$\dev$          \\
% \midrule
% Cross entropy &  61.94($\pm$0.28)              &    27.13($\pm$0.35)         &  55.59($\pm$0.26)              &   29.10($\pm$0.64)       &43.76($\pm$0.74) & 31.69($\pm$0.81) \\
%  $\nodic_{\text{Bilevel}}$ (AutoBalance \cite{li2021autobalance})     &  56.70($\pm$0.32)              &    20.13($\pm$0.68)         &  50.93($\pm$0.16)              &   26.06($\pm$0.61)      &40.04($\pm$0.79) &   36.30($\pm$0.89)    \\
%  $\name_{\text{Bilevel}}$: $\att_{\textsc{freq}}$     &  56.64 ($\pm$0.21)             &    19.10($\pm$0.67)         &  50.82($\pm$0.13)               &   24.36($\pm$0.49)       & 39.91($\pm$0.66)&  26.54($\pm$0.80)    \\
%                            $\name_{\text{Bilevel}}$: $\att_{\textsc{diff}}$     &  58.27($\pm$0.24)              &   \textbf{17.62}($\pm$0.65)             &     52.97($\pm$0.30)  &           \textbf{21.28}($\pm$0.58)       & 40.61($\pm$0.61)&  \textbf{14.49}($\pm$0.72)   \\
%                            $\name_{\text{Bilevel}}$: $\att_{\textsc{freq}}$+$\att_{\textsc{diff}}$  &   \textbf{56.38}($\pm$0.19)             &     18.53($\pm$0.63)           &    \textbf{49.31}($\pm$0.34)            &  22.14($\pm$0.46)            & \textbf{38.36}($\pm$0.79)&
% 19.78($\pm$0.75) \\
% \bottomrule
% 		\end{tabular}}\vspace{-10pt}\caption{Attributes help optimization adapt to dataset heterogeneity. We conduct experiments using bilevel loss design and report the balanced misclassification error,and standard deviation of class-conditional errors with different class-specific attributes.}\label{table:attributes_lt}\vspace{-10pt}

% \end{table*}



\subsection{Benefits of \name for Adapting to Distinct Class Heterogeneities}\label{sec:attribute}
Continuing the discussion in Sec.~\ref{sec:attributes}, we investigate the advantage of different attributes in the context of dataset heterogeneity adoption. In  Table~\ref{table:attributes_lt}, we conduct loss function design $\name$ experiments on CIFAR-LT and ImageNet-LT dataset. Specifically, besides using regular CIFAR100-LT and ImageNet-LT, we introduce label noise into CIFAR10-LT following \cite{tanaka2018joint,reed2014training} to extend the heterogeneity of the dataset. To add the label noise, firstly, we split the training dataset to 80\% train and 20\% validation to accommodate bilevel optimization. Then we randomly generate a noise ratio $\bm{r}\in \R^K, \bm{r}_i \sim U(0,0.5)$ that denotes the label noise ratio for each class. Finally, keeping the validation set clean, we add label noise into the train set by randomly flipping the labels of selected training samples (according to the noise ratio) to all possible labels. As a result, all classes contain an unknown fraction of label noise in the noisy CIFAR10-LT dataset, which raises more heterogeneity and challenge in optimization. Through bilevel optimization, we optimize the balanced classification loss and report the balanced test error and its standard deviation after the retraining phase in Table~\ref{table:attributes_lt}. As shown in Table~\ref{table:attributes_lt}, we employ label frequency $\attfreq$ which is designed for sample size heterogeneity and $\attdiff$ which is designed for class predictability as the attributes in $\name$ approach. Table~\ref{table:attributes_lt} highlights that $\name$ consistently outperforms other methods while different attributes can shape the optimization process differently. Importantly, CAP is particularly favorable to tail classes which contain too few examples to optimize individually. Only using $\attdiff$ achieves smallest $\dev$ demonstrating that optimization with $\attdiff$ tends to keep better class-wise fairness because $\attdiff$ is directly related to class predictability. The combination of $\attfreq$ and $\attdiff$ shows that incorporating multiple class-specific attributes provides additional information about the dataset and jointly enhances performance. Overall, the results indicate that $\name$ establishes a principled approach to adapt to multiple kinds of heterogeneity.
% \noindent\textbf{CAP improves the performance of diverse fairness objectives.} Table~\ref{table:attributes_objective} shows the benefit of attributes for optimizing different fairness objectives when we use post-hoc $\name$. In this table, $\berr, \dev, \quan, \cv$ are different fairness criteria based on error statistics as detailed in Sec.~\ref{sec:objective}.  $\werr$ denotes a weighted test objective induced by weights $\bm{\omega}^{\text{test}}_k\in\R^K$ given by\vspace{-0pt}
% \begin{align}
% \vspace{-20pt}
%     \werr=\sum_{k=1}^{K}{\bm{\omega}^{\text{test}}_k\err_{k}}\quad\text{where}\quad \sum_{k=1}^K\bm{\omega}^{\text{test}}_k=K.\label{weighted obj}
%     \vspace{-20pt}
% \end{align} We report the average result of 10 trails of different $\bm{\omega}^{\text{test}}$ for $\werr$. At each trial, weights $\bm{\omega}^{\text{test}}_k$ are generated i.i.d.~from the uniform distribution over $[0,1]$. We consider the three attributes highlighted in Table \ref{table:attributes_definition}, namely $\attfreq,\attdiff,\attw$. For each test objective, we report the single best attribute as well as combination of all attributes. 

% %For the attributes, in Table~\ref{table:attributes_objective}, we select the one or two attributes from $\attfreq,\attdiff,\attw$ that achieves best objective performance for single attribute and combined attribute respectively. With one attribute, $\berr,\werr$ prefer  and $\dev,\cv,\quan$ prefers $\attdiff$. 
% We found that the best attribute for $\berr,\werr$ are $\attfreq$ and for $\dev,\cv,\quan$ are $\attdiff$. Observe that $\attw$ is not informative for unweighted objectives $\berr,\dev,\cva{0.2},\quana{0.2}$, thus these only use $\attfreq$ and $\attdiff$ for the ``All attributes'' row.
% %for achieving best performance. But for $\werr$, the combination of $\attfreq$ and $\attw$ outperforms other combinations. This selection is also consist with Theorem 1 of \cite{menon2020long} where logit adjusted loss requires $\attfreq$ and $\attw$ to be Fisher consistent. 
% Overall, Table~\ref{table:attributes_objective} shows that $\name$ with all attributes consistently achieve the best results on multiple fairness objectives. For the $\name$ with single attribute, the best attribute varies with the test objective, which demonstrates the flexibility of $\name$ strategy. An important conclusion is that, benefit of CAP is more significant for objectives beyond balanced accuracy and improvements are around 2\% or more (compared to \cite{menon2020long} or plain post-hoc). This is perhaps natural given that prior works put an outsized emphasis on balanced accuracy in their algorithm design  \cite{menon2020long,li2021autobalance}.

% \textbf{Implementation}  
% The benefits of dictionary attributes was shown in three different scenarios. In setting A, we use bilevel optimization to design the loss function and show the final result after retraining. The objective is the balanced error. This experiment shows the benefits of $\name$ on natural datasets with predictability and sample size heterogeneities. In setting B, we use the same optimization strategy as setting A, but we conduct the experiment on the imbalance dataset with noisy labels. The takeaway of this experiment is to present the flexibility of $\name$ in different heterogeneities. To generate a dataset with class frequency and label quality heterogeneities, we add noisy labels to the long-tailed CIFAR10. Following previous works \cite{tanaka2018joint,reed2014training}, we experiment with symmetric label noise. The label noise is generated by randomly flipping the labels of selected training samples to all possible labels. We still split the long-tailed training set into 80\% training and 20\% validation. We keep the validation dataset clean. For training dataset, a random noise ratio $\text{r} = N_{noisy} / N_{total} \in [0,0.5]$ was generated for each class. In setting C, we use post-hoc adjustment to adapt various fairness objectives efficiently and compare them with SOTA approaches. From those three experiments, we propose that multiply choices of attributes provide flexibility, which could outperform prior art and show significant improvements in different scenarios.\\  

% In setting C the result was adjusted via post-hoc while in setting A we search the best loss via bilevel training. $\att_{freq}$ is the class frequency and $\att_{diff}$ is the class-conditional risks$\err_{k}(f)$ for pretrained model. $\att_{weight}$ is the target class weight for weighted class error $\werr$. In setting B, we use $\name_{\text{AB}}$ without initialization and with 120 epoches warm-up. $\att_{freq}$ is the frequency of original labels, which is the same as it in class imbalance setting $\mathbb{A}_{freq} = normalized(N_{y} / N_{max})$. We add $\att_{diff}= normalized(\text{class error})$ to adapt noisy label. Class error was computed at the end of warm-up.\\
		
%\textbf{Results and discussion} 
%Table\ref{table:attributes_lt} shown the results of setting A and B. We compare two different attributes $\att_{\text{freq}}$ which is designed for sample size heterogeneities and $\att_{\text{diff}}$ which is designed for class predictability. High average performance doesn't always mean high fairness. We also evaluate using standard deviation$\dev$, which quantifies fairness directly. Comparing the results, $\name$ could always outperform other methods. Simply using $\att_{\text{diff}}$ could get the smallest standard deviation but couldn't decrease balanced error a lot. Although $\name$ with only $\att_{\text{freq}}$ is able to achieve high average performance, it also increases the standard deviation, which means that it actually sacrifices some low predictability classes and causes unfairness. After adjusting using $\att_{\text{diff}}$, the worst classes are not the smallest class anymore. So other reasons cause low predictability, and only $\att_{\text{freq}}$ is hard to adjust. In setting A, it might cause by indistinct property and high semantic similarity among classes. In setting B, which use the dataset with noisy labels, label quality is one of the reasons. By combining attributes, $\name$ could deal with heterogeneities caused by different reasons and achieve low balanced error$\berr$ and standard deviation$\dev$ simultaneously.\\

%Table\ref{table:attributes_objective}, we compare attributes for different fairness objectives. Same as the results in setting A and B, $\name$ combining features could always achieve best results. Comparing $\name$ with single attributes$\att$, the best attributes varies according to the objectives. 

%For $\dev$, which quantifies the similarly for class-conditional errors, $\quan$ and $\cv$ ,which focus on errors on different target classes, $\att_{\text{diff}}$ could achieve better result. For objectives evaluate weighted performance, balanced error is one of the special case, $\att_{\text{freq}}$ is the best.


% In Table\ref{table:attributes_objective}, we compare attributes for different objectives. For all settings, combining attributes outperforms using single attributes. Which attributes are better varies according to the objectives.




		
% \vspace{-10pt}
% \subsection{Experiment details and reproducibility}\label{sec:detail}
% \vspace{-5pt}
% \mli{@TODO: We can move this part to Appendix for more space}

% % \mli{Fix function value choice here}
% % In our experiments, $\bm{\Func}$ varies by the dataset, for CIFAR10-LT, we use $\bm{\Func}=[\log(\att),\att^{-1},\att^{0.3}]$. For CIFAR100-LT, $\bm{\Func}=[\log(\att),\att^{-1},\att^{0.15}]$, and for ImageNet-LT we have $\bm{\Func}=[\log(\att),\att^{-1},\att^{0.075}]$. We remark that to be consistent in the same dataset, the functions are fixed for each dataset regardless of the objectives change.
% \xuechen{The functions are always fixed regardless of the datasets and objectives change $\bm{\Func}=[\log(\att),\att,\att^{\beta},\att^{2\beta},\att^{4\beta}]$. In our experiments, we set $\beta = 0.075$.}

% \xuechen{For reproduced result in Table~\ref{table:dic}, we grid search on validation dataset and retrain for fair comparison, so the result is worse than the value reported in \cite{menon2020long,ye2020identifying} which are grid searched on whole test dataset.}
% %We remark that to be consist in the same dataset, the functions are fixed for each dataset regardless the change of objectives.
% % For post-hoc training, we add early-stopping. In \ref{table:posthoc}, to avoid $\boldsymbol{l}$\&$\boldsymbol{\Delta}$ canceling out each other during the training, we first optimize $\boldsymbol{l}$ for 200 epoch then fix $\boldsymbol{l}$ value and start optimizing $\boldsymbol{\Delta}$ for another 200 epoch. Considering about the results in \ref{table:posthoc}, $\boldsymbol{\Delta}$ doesn't help and even hurt the result.  In all the other post-hoc adjustment experiments, we only use $\boldsymbol{l}$ for better performance. As post-hoc doesn't need high computational resources, we could use a larger batchsize which is 256 in this paper. 

% For bilevel training, following the training process in  \cite{li2021autobalance}, we start the validation optimization after 120 epochs warmup and training 300 epochs in total. The learning rate decays at epochs 220 and 260 by a factor 0.1. The lower-level optimization use SGD with an initial learning rate 0.1, momentum 0.9, and weight decay $1e-4$, over 300 epochs. At the same time, the upper-level hyper-parameter optimization also uses SGD with an initial learning rate 0.05, momentum 0.9, and weight decay $1e-4$. To get better results, we initialize $\boldsymbol{l}$ using LA loss in experiments in Table~\ref{table:dic}. For a fair comparison, there is no initialization in other experiments. For LA and CDT results in Table~\ref{table:dic}, we do grid search on the imbalanced validation dataset and retrain for a fair comparison.

% For most of the experiments, except $\werr$ in Table~\ref{table:attributes_objective}, we plot or report the average result of 3 runs. For $\werr$ where the target weight $\bm{\alpha}$ was generated randomly, we repeat ten times with different random seeds. 

% \xuechen{For LA and CDT result in Table~\ref{table:dic}, we do grid search on imbalanced validation and retrain for fair comparison.}

% \xuechen{For attributes comparison results in Table~\ref{table:attributes_objective}, we use attributes $\att = [\attfreq ,\attdiff, \attw]$. For objectives except $\werr$, the $\attw$ are all ones.}
% 		\begin{table}
% 	\begin{center}%\resizebox{\textwidth}{!}{
% 			\begin{tabular}{llllll}
% 				\toprule
% %\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
% %\toprule
% \multicolumn{1}{l}{Post-hoc methods}                  & $\berr$              & $\dev$ & $\cva{0.2}$ &$\quana{0.2}$ &$\werr$ \\
% \midrule
% Baseline (\pretrain~model)&        61.94        & 27.13  & 96.95  &  93.01 &62.53 \\
%   $\nodic$ post-hoc    &    -1.62            & -4.89  & -6.41  & -10.28 &-2.30  \\
%   $\text{Logit-adjustment}$ of \cite{menon2020long} &       -3.73        & -9.53  & -10.21  & -14.79 &  -2.84 \\
%  $\name$: Single best attribute     &    -4.23           & \textbf{-12.77}  & -9.85  & -14.82 & -3.79  \\
%  %$\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
%  $\name$: All attributes &  \textbf{-4.36}   &  \textbf{-12.78}  & \textbf{-12.02}  & \textbf{-16.98} & \textbf{-5.42}\\



==> sec/methods.tex <==
%!TEX root = ../automl.tex
\vspace{-4pt}
\section{Our Approach: Class-attribute Priors (\name)}\label{sec:cap}
		\begin{table*}
	\begin{center}\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llll}
\toprule
 Attributes            & Definition &Notation& Application scenario \\
\midrule
\red{ $\att_{\textsc{freq}}$}         & Class frequency & $\pi_k=\Pro(y=k)$& Imbalanced classes\\
 \red{$\att_{\textsc{diff}}$ }        & Class-conditional error & $\Pro(y\neq \hat{y})$& Difficult vs easy classes\\
 \red{$\att_{\textsc{weights}}$}      & Test-time class weights & $\omega^{\text{test}}_k$ of \eqref{weighted obj}& Weighted test accuracy\\
 \midrule
 $\att_{\textsc{noise}}$ & Label noise ratio & $\Pro(y^{\textsc{clean}}\neq y\big|y^{\text{clean}}=k)$ & Datasets with label noise\\
 $\att_{\textsc{norm}}$ &  Norm of classifier weights & See \cite{cao2019learning} & Imbalanced classes\\
  %... & ...  & ...\\
\bottomrule
		\end{tabular}}\vspace{-3pt}\caption{Definition of example attributes and associated application scenarios. Attributes $\attdiff$ and $\attnorm$ are computed during the training (for post-hoc optimization, it is pre-training). For bilevel training they are computed at the end of warm-up. The upper attributes in \red{red} color are those we utilize in our experiments. Also we use \red{$\Ac_{\textsc{all}}$} to denote combined attributes. }\label{table:attributes_definition}
	\end{center}
		\end{table*}
% \iffalse
% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% method                         & phase1:initialization     & phase2:search phase & phase3:retrain & final result \\ \hline
% autobalance                    &simple training & bilevel             & retrain(tuned loss)        &              \\ \hline
% autobalance(dic)               &simple training & bilevel(dic)        & retrain(tuned loss)        &              \\ \hline
% autobalance(dic)               & /                         & bilevel(dic)        & retrain(tuned loss)        &              \\ \hline
% post-hoc                       &simple training & /                   & post-hoc       &              \\ \hline
% post-hoc transfer              &simple training & post-hoc            & retrain(tuned loss)        &              \\ \hline
% self-sup                       & Simsiam                   & /                   & retrain(wCE, LA loss)        &              \\ \hline
% self-sup bilevel               & Simsiam                   & bilevel             & retrain(tuned loss)        &              \\ \hline
% simple training initialization & simple training & /                   & retrain(wCE, LA loss)         &              \\ \hline
% \end{tabular}
% \end{table}
% \fi


% \begin{table}[t]
% 	\small
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lccccc}
% 				\toprule
% 				& CE, 100 epoch & CE, 120 epoch & CE, 200 epoch &LA, 120 epoch & Self-sup \\
%               \toprule
%               Std when search phase begin & 0.23 &      0.20  & 0.28 &        0.17  &  0.13 \\
% 				\midrule
% 				Balanced accuracy & 24.58 & 21.39      &  23.36 & 21.15         & 20.57  \\
% 				\bottomrule %\vspace{10pt}
% 		\end{tabular}}\caption{Bilevel training with different warm-up lead to different result. 120 epochs Warm-up with CE or LA loss are used in autobalance paper. paper(\cite{li2021autobalance}).}\label{table:warmup_result}\vspace{-10pt}
% 	\end{center}
% \end{table}

We start with a motivating question:

\emph{\textbf{Q:} Does utilizing multiple class attributes provably help?}

To answer this, we consider the benefits of multiple attributes for a binary gaussian mixture model (GMM) and provide a simple theoretical justification why synergistically leveraging attributes can help balanced accuracy. Consider a GMM where data from the two classes are generated as
\begin{align*}
y = \begin{cases} +1 &,\text{with prob.}~\pi
\\
-1 &,\text{with prob.}~1-\pi
\end{cases}
~~~\text{and}~~~\mathbf{x}|y\sim \mathcal{N}(y\boldsymbol{\mu},\sigma_y\mathbf{I}_d).
\end{align*}
Note here that the two classes are \textbf{imbalanced} as a function of the value of $\pi\in(0,1)$, which models class frequency. Also, the two classes are allowed to have different noise variances $\sigma_{\pm1}$. This is our model for the \textbf{difficulty} attribute: examples generated from the class with larger variance are ``more difficult" to classify as they fall further apart from their mean. Intuitively, a ``good" classifier should account for both attributes. We show here that this is indeed the case for the model above. Our setting is as follows: Draw $n$ IID samples $(\mathbf{x}_i,y_i)$ from the GMM distribution above. Without loss of generality, assume class $y=+1$ is minority, i.e. $\pi<1/2$. We train linear classifier $(\mathbf{w},b)$ by solving the following cost-sensitive support-vector-machines (CS-SVM) problem:
\begin{align*}
(\hat{\mathbf{w}}_\delta,\hat{b}_\delta):=\arg\min_{\mathbf{w},b} \|\mathbf{w}\|_2~\text{s.t.}~y_i(\mathbf{x}_i^T\mathbf{w}+b)\geq\begin{cases}
    \delta & y_i=+1
    \\
    1 & y_i=-1
    \end{cases}.
\end{align*}
Here, $\delta$ is a hyperparameter that when taking values larger than one, it pushes the classifier towards the majority, thus assigning larger margin to the minorities. In particular, setting $\delta=1$ recovers the vanilla SVM. CS-SVM is particularly relevant to our setting because it has rigorous connections to the generalized cross-entropy loss in Sec \ref{loss func} (see Appendix F for details). %is that it relates closely to the VS-loss. Specifically,  \cite{kini2021label} show that in linear overparameterized (aka $d>n$) settings the VS-loss with multiplicative weights $\Delta_\pm1$ leads to same performance as the CS-SVM with $\delta=\Delta_+/\Delta_-.$ 
Given CS-SVM solution $(\hat{\mathbf{w}}_\delta,\hat{b}_\delta)$, we measure the balanced error as follows:
$$
\mathcal{R}_{\text{bal}}(\delta):= \mathbb{P}_{(\mathbf{x},y)\sim\text{GMM}}\left\{y(\mathbf{x}^T\hat{\mathbf{w}}_\delta+\hat{b}_\delta)>0\right\}.
$$
We ask: How does the optimal CS-SVM classifier (i.e, the optimal hyperparameter $\delta$) depend on the data attributes, i.e. on the frequency $\pi$ and on the difficulty $\sigma_{+1}/\sigma_{-1}$? To answer this we consider a high-dimensional asymptotic setting in which $n,d\rightarrow\infty$ at a linear rate $d/n=:\bar{d}$. This regime is convenient as previous work has shown that the limiting behavior of the balanced error $\mathcal{R}_{\text{bal}}(\delta)$ can be captured precisely by analytic formulas \cite{montanari2019generalization}. Specifically, \cite{kini2021label} computes formulas for the optimal hyperparameter $\delta$ when $\pi$ is variable but both classes are equally difficult, i.e. $\sigma_{+1}=\sigma_{-1}$. Here, we derive risk curves for arbitrary $\sigma_{\pm 1}$ by extending their study and investigate the synergistic effect of frequency and difficulty.

Figure \ref{fig:gmmm} confirms our intuition: \textbf{the optimal hyperparameter $\delta_*$ (y-axis) does indeed depend on the frequency and difficulty} (as well as the training sample size, x-axis). Specifically, we observe in both Figures \ref{fig:gmmm}(a,b) that as the minority class becomes easier (aka, the smaller ratio $\sigma_{+1}/\sigma_{-1}$), $\delta$ decreases. That is, there is less need to assign an even larger margin for the minority. Conversely, as $\sigma_{+1}/\sigma_{-1}$ increases and minority becomes more difficult, its margin gets a boost. Finally, comparing Figures \ref{fig:gmmm}(a) to \ref{fig:gmmm}(b), note that $\delta_*$ takes larger values for larger imbalance ratio (i.e., smaller frequency $\pi$), again aggreeing with commonsense. 

Since GMM data is synthetic, $\delta_*$ can be computed analytically. Our approach \name will facilitate realizing such benefits systematically and efficiently for arbitrary class attributes.

% \begin{figure}[h]
% \centering
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.3]{\includegraphics{./figs/gmm.eps}};
% 	\end{tikzpicture}\vspace{-4pt}\caption{$\name_{\text{Post-hoc}}$:The optimal hyperparameter depends on both attributes: frequency and difficulty.}
% \end{figure}

\begin{figure}
\begin{subfigure}{1.54in}
\includegraphics[scale=0.218]{./figs/gmm_1.pdf}
 \caption{Imbalance $\pi=0.1$}
\end{subfigure}~
\begin{subfigure}{1.54in}
\includegraphics[scale=0.218]{./figs/gmm_2.pdf}
 \caption{Imbalance $\pi=0.2$}
\end{subfigure}
\caption{The optimal hyperparameter $\delta_*$ depends on both attributes: frequency ($\pi$) and difficulty ($\sigma_+/\sigma_-$).}
\label{fig:gmmm}
\end{figure}

\subsection{Attributes and Adaptation to Heterogeneity}\label{sec:attributes}
%\som{start with the example of posthoc adjustment}
{To proceed, we introduce our \name approach at a conceptual level and  provide concrete applications of \name to loss function design in the next section.} Recall that our high-level goal is designing a map from $\Strat$ that takes attributes $\att_k$ of class $k$ and generates the hyperparameters of the optimization strategy $\strat_k$. Each coordinate $\att_k[i]$ characterizes a specific attribute of class $k$ such as label frequency, label noise ratio, training difficulty shown in Table~\ref{table:attributes_definition}. To model $\Strat$, one can use any hypothesis space including deep nets. However, since $\Strat$ will be optimized over the validation loss, depending on the application scenario, it is often preferable to use a simpler linearized  model.

\noindent\textbf{Linearized approach.} Suppose each class has $n$ attributes with $\att_k\in\R^n$. We will use a nonlinear feature map $\bm{\Func}(\cdot):\R^n\rightarrow \R^M$ where $M$ is the embedding space. Suppose the class-specific strategy $\strat_k\in\R^s$. Then, $\Strat$ can be parameterized by a weight matrix $\W\in\R^{s\times M}$ so that
\begin{align}
\vspace{-15pt}
\strat_k = \Strat(\att_k):=\W\bm{\Func}(\att_k).\label{Wmap}
\vspace{-15pt}
\end{align}
Our goal becomes finding $\W$ so that the resulting strategies maximize the target validation objective. Observe that $\W$ has $s\times M$  parameters rather than $s\times K$ parameters which is the naive approach that learns individual strategies. In practice, $K$ can be significantly large, so for typical problems, $M\ll K$. Moreover, $\W$ ties all classes together during training through weight-sharing whereas the naive approach would be brittle for tail classes that contain very limited data. 
%The approach are summarized in Fig.~\ref{fig:a2h}

\subsection{\name for Loss Function Design}\label{loss func}
%\mli{This paragraph is very confusing, especially W and $\Dic$} 

Consider the generalized cross-entropy loss \[
\ell(y, f(\x))=\omega_y\log (1+\sum_{k \neq y} e^{\lb_{k}-\lb_{y}} \cdot e^{\Deltab_{k} f_{k}(\x)-\Deltab_{y} f_{y}(\x)}).
\]
Here, $(\omega_k,\lb_k,\Deltab_k)_{k=1}^K$ are hyperparameters that can be tuned to optimize the desired test objective. For class $k$, we get to choose the tuple $\strat_k:=[\omega_k,\lb_k,\Deltab_k]$ which can be considered as its training strategy. Here elements of $\strat_k$ arise from existing imbalance-aware strategies, namely weighting $\omega_k$, additive logit-adjustment $\lb_k$ and multiplicative adjustment $\Deltab_k$.

\noindent\textbf{Example: LA and CDT losses viewed as \name.} For label imbalanced problems, \cite{menon2020long,ye2020identifying} propose to set hyperparameters $\lb_k$ and $\Deltab_k$ as a function of frequency $\pi_k=\Pro(y=k)$. Concretely, they propose $\lb_k=-\gamma\log(\pi_k)$ \cite{menon2020long} and $\Deltab_k=\pi_k^\gamma$ \cite{ye2020identifying} for some scalar $\gamma$. These can be viewed as special instances of \name where we have a single attribute $\Ac_k=\pi_k$ and $\Strat(x)$ is $-\gamma\log(x)$ or $x^\gamma$ respectively.

%Observe that $k$'th classes strategy is dictated by the variables $\strat_k=[w_k,\lb_k,\Deltab_k]$.

\noindent\textbf{Our approach} can be viewed as an extension of these to attributes beyond frequency and general class of $\Strat$. In light of \eqref{Wmap}, hyperparameters of a specific element of $\strat_k=[\omega_k,\lb_k,\Deltab_k]$ correspond to a particular row of $\W\in\R^{3\times M}$ since $\W=[\w_{\bm{\omega}},\w_\lb,\w_\Deltab]^\top$. Our goal is then tuning the $\W$ matrix over validation data. In practical implementation, we define a feature dictionary 
\begin{align}
\vspace{-20pt}
\Dic = \begin{bmatrix}\bm{\Func}(\att_1)~\cdots~\bm{\Func}(\att_K)\end{bmatrix}^\top \in \mathbb{R}^{K\times M}.\label{dicdic}
\vspace{-20pt}
\end{align}
Each row of this dictionary is the features associated to the attributes of class $k$. We generate the strategy vectors $\Deltab, \lb,\bm{\omega}\in\R^K$ (for all classes) via $\bm{\omega}=\Dic\w_{\bm{\omega}}$, $\Deltab=\text{sigmoid}(\sqrt{K}\frac{\Dic\w_\Deltab}{\|\Dic\w_\Deltab\|})$, $\lb=\Dic\w_\lb$.
%\mli{Confused with the dimension here, can we discuss?} We can then generate the global strategy vectors (per-element) via  \mli{Should we include weights $w$ in this example, since we didn't use it anywhere in other parts}

%\noindent\textbf{Example: }
For both loss function design and post-hoc optimization, we use a decomposable feature map $\bm{\Func}$. Concretely, suppose we have basis functions $(\Func_i)_{i=1}^m$. These functions are chosen to be poly-logarithms or polynomials inspired by \cite{menon2020long,ye2020identifying}. For $i$th attribute $\att_k[i]\in\R$, we generate $\bm{\Func}(\att_k[i])\in\R^m$ obtained by applying $(\Func_i)_{i=1}^m$. We then stitch them together to obtain the overall feature vector $\bm{\Func}(\att_k)=[\bm{\Func}(\att_k[1])^\top~\cdots~\bm{\Func}(\att_k[m])^\top]\in\R^{M:=m\times n}$. We emphasize that prior approaches are special instances where we choose a single basis function and single attribute $\pi_k$.% (namely $\pi_k$).

%Overall $\name$ generates a class-specific strategy based on its attributes. As we shall demonstrate in experiments, CAP flexibly adapts to various types of objectives and heterogeneities. Besides benefiting sample efficiency and generalization, it also improves the training process by reducing instability of hyperparameter optimization and accelerating training.


%, and boosts the generalization performance on the imbalanced datasets. 
%We introduce a dictionary design to ease up the influence of heterogeneity on the learning process. Formally, we define the attribute $\att \in \mathbb{R}^{K \times n}$ contains $n$ different attributes, where each attribute $\att_i$ characterize a specific attribute for $K$ classes such as label frequency, label noise ratio, training difficulty shown in Table.~\ref{table:attributes_definition}. Then let $\bm{\Func}=[\Func_1, \Func_2, ..., \Func_m]$ denotes $m$ functions that normalize $\att$ to match the scope of $\lb,\Deltab$ (e.g. logarithm or polynomial functions).
%We define \dictionary as $\Dic = \bm{\Func}(\att) \in \mathbb{R}^{K\times mn}$ which applies all functions on all attributes. 
%Let $\w_\lb,\w_\Deltab \in \mathbb{R}^{mn}$ denote the weighting of \dictionary vectors for $\lb$ and $\Deltab$ respectively. In out paper, $\name$ strategy is implemented in the dictionary design as $\Strat=[\Dic \w_\lb, \Dic \w_\Deltab]$ where we optimize $\w_\lb$ and $\w_\Deltab$ and fix $\Dic$. So the dimensions of outer problem reduces to $2mn$ for only optimizing $\w_\lb$ and $\w_\Deltab$. The benefits can be introduced in two aspects. Firstly, $\name$ proposes a class-specific strategy based on its attributes. Its flexibility could adapt to various objectives and types of imbalance. Secondly, it improves the training process by reducing instability on bi-level optimization, accelerates training, and boosts the generalization performance on the imbalanced datasets. 
% 		\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{
% \begin{tabular}{lll}
% \toprule
%  Attributes            & Definition & scenarios \\
% \midrule
%  $\att_{\text{freq}}$         & class frequency & Designed for imbalance datasets.\\
%  $\att_{\text{diff}}$         & \makecell[l]{predictability (easy vs difficult),\\ computed as class-conditional risks} & \makecell[l]{Overweight bad-performance classes. \\Could be used without knowing the type of imbalance. \\ Performs good for target classes related objectives.}\\
%  $\att_{\text{weights}}$      & \makecell[l]{variable importance at test-time,\\ computed as new weights for target distribution} & Designed for distribution shift.\\
%  $\att_{\text{noisy}}$ & label quality, \makecell[l]{computed as noise ratio of each class} & Designed for datasets with noisy label.\\
%  $\att_{\text{norm}}$ &  norm of the weight vectors of the last fully-connected layer & \makecell[l]{Label-distribution-aware value. \\Could be used without knowing class}\\
%   ... &   & \\
% \bottomrule
% 		\end{tabular}}\caption{Definition and scenarios\xuechen{rethink. writing issue}}\label{table:attributes_definition}\vspace{-6pt}
% 	\end{center}
% 		\end{table}

% 		\begin{table*}
% 	\begin{center}\resizebox{0.8\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%  Attributes            & Definition &Notation& Application scenario \\
% \midrule
% \red{ $\att_{\textsc{freq}}$}         & Class frequency & $\pi_k=\Pro(y=k)$& Imbalanced classes\\
%  \red{$\att_{\textsc{diff}}$ }        & Class-conditional error & $\Pro(y\neq \hat{y})$& Difficult vs easy classes\\
%  \red{$\att_{\textsc{weights}}$}      & Test-time class weights & $\omega^{\text{test}}_k$ of \eqref{weighted obj}& Weighted test accuracy\\
%  \midrule
%  $\att_{\textsc{noise}}$ & Label noise ratio & $\Pro(y^{\textsc{clean}}\neq y\big|y^{\text{clean}}=k)$ & Datasets with label noise\\
%  $\att_{\textsc{norm}}$ &  Norm of classifier weights & See \cite{cao2019learning} & Imbalanced classes\\
%   %... & ...  & ...\\
% \bottomrule
% 		\end{tabular}}\vspace{-3pt}\caption{Definition of example attributes and associated application scenarios. Attributes $\attdiff$ and $\attnorm$ are computed during the training (for post-hoc optimization, it is pre-training). For bilevel training they are computed at the end of warm-up. The upper attributes in \red{red} color are those we utilize in our experiments. Also we use \red{$\Ac_{\textsc{all}}$} to denote combined attributes. }\label{table:attributes_definition}
% 	\end{center}
% 		\end{table*}
\noindent\textbf{Which attributes to use and why multiple attributes help?} Attributes should be chosen to reflect the heterogeneity across individual classes. These include class frequency, difficulty of prediction, noise level and more. We list such potential attributes $\att$ in Table~\ref{table:attributes_definition}. The frequency $\attfreq$ is widely used to mitigate label imbalance, and $\attnorm$ is inspired by the imbalanced learning literature~\cite{cao2019learning}. However, these may not fully capture the heterogenous nature of the problem. As discussed above for GMMs (Fig \ref{fig:gmmm}), some classes can be more difficult to learn and require more upweighting despite containing sufficient training examples. This motivates the use of $\attdiff$. Moreover, rather than balanced accuracy, we may wish to optimize general test objectives including weighted accuracy with varying class importance. We can declare these test-time weights as an attribute $\attw$. Appendix provides theoretical justification for incorporating $\attw$ by showing \name can accomplish Bayes optimal logit adjustment for weighted error. More broadly, any class-specific meta-feature can be used as an attribute within \name. 
%and how CAP accomplishes this.
%needed for a Gaussian Mixture dataset model.
%\noindent\textbf{Why multiple attributes help?} In Section \ref{app:gmm}, 
%there is still a large potential to discover and design new attributes.

%Such prior information
%may be h some  such as target class importance that can be treated as . 


% For function $\Func$, we use log function, polynomial function $\att^\gamma$ with several power values. In this paper, we commonly use power value $\gamma \in [-1,0.075,0.15,0.3]$. The selection of functions varies based on datasets, search space, objectives, etc..   \mli{We can remove this paragraph because it is redundant to prior paragraphs}

\noindent\textbf{Reduced search space and increased stability.} Searching $\lb$ and $\Deltab$ on $\mathbb{R}^{K}$ with very few validation samples raises the problem of unstable optimization. \cite{li2021autobalance} indicates the bilevel optimization is brittle and hard to optimize. They introduce a long warm-up phase and aggregate classes with similar frequency into $g$ groups, reducing \red{the} search space to $k/g$ dimensions. However, to achieve a fine-grained loss function, $g$ cannot be very large, so the search space remains large. In our method, with a good design of $\Dc$ (normally $n\approx 2$ and $m\approx 3$), we can utilize a constant $2mn\ll K$ that efficiently reduces the search space and provides better convergence and stability.

We remark that \dictionary is a general and efficient design that can recover multiple existing successful imbalanced loss function design algorithms. For example, \cite{menon2020long} and \cite{ye2020identifying} both utilize the frequency as $\att$ and apply logarithm and polynomial functions as $\Func$ on frequency to determine $\lb$ and $\Deltab$ respectively. Moreover, let $\att=\bm{I}_k$ and $\Func$ be an identity function, then training $\w_\lb, \w_\Deltab$ is equivalent to train $\lb,\Deltab$ which recovers the algorithm of \cite{li2021autobalance}. Despite the ability to generalize, the \dictionary is more flexible and powerful since the attributes can be chosen based on the scenarios. For example, naturally, class frequency is a critical criterion in an imbalanced dataset, but classification error in early training can also be a good criterion for evaluating class training difficulty. Furthermore, some specific attributes can be introduced to noisy or partial-labeled datasets to help design a better loss function. Our empirical study elucidates the benefit of combining multiple attributes and the \dictionary performance on the noisy imbalanced dataset.

% In our experiments, we use frequency $\att_{\text{freq}}$ inspired by \cite{ye2020identifying} and \cite{menon2020long}, difficulty $\att_{\text{diff}}$ which is related to the class error in early epochs of training, the norms of the classifier weights $\att_{\text{weight}}$ inspired by \cite{kang2019decoupling}; For function $\Func$, we use polynomial and logarithm function inspired by \cite{ye2020identifying,menon2020long}.
% \xuechen{objective? more stable? only update target classes?}
% \mli{HERE}

% We use the attributes $\mathbb{A}$ which are related to information such as class frequency, noisy ratio, and class error. The attribute could be choose based on the scenarios. Naturally, class frequency could be used when there are class-frequency-imbalance and class error could be used when some class is more difficult to train. In many scenarios, class frequency is not the only reason of imbalance. For example, for dataset with noisy label noisy ratio also influence the training. Bias is not always easy to quantify. The reason might be complex and be the cross term of several factors. Several attributes could be used at the same time and dictionary should combine those automatically.




% The benefits can be introduced in two aspects. (1) Introducing the prior information could help adjust training loss. This is demonstrated by CDT loss in \cite{ye2020identifying} and LA loss in \cite{menon2020long} which introduce the prior of class y to adjust training loss and outperformed other heuristics (e.g., focal loss \cite{lin2017focal}). But using a single function of prior information is not enough. Paper\cite{menon2020long} mentioned that combining their relative margin with the adaptive margin could achieve better result on on iNaturalist. (3)An important challenge of AutoBalance training is the dimensionality of hyperparameter.

% We propose subspace-based search spaces for hyperparameters. We use the attributes $\mathbb{A}$ which are related to information such as class frequency, noisy ratio, and class error. The attribute could be choose based on the scenarios. Naturally, class frequency could be used when there are class-frequency-imbalance and class error could be used when some class is more difficult to train. In many scenarios, class frequency is not the only reason of imbalance. For example, for dataset with noisy label noisy ratio also influence the training. Bias is not always easy to quantify. The reason might be complex and be the cross term of several factors. Several attributes could be used at the same time and dictionary should combine those automatically. 

% To use the attributes as weights, we use functions $\mathbb{F}$ which could help the attributes value adapt to different hyperparameters. For example log function is used for $l$ in LA loss while polynomial is used for $\Delta$ in CDT loss. The functions and attributes compose dictionary $\boldsymbol{D} = \mathbb{F}(\mathbb{A})$. $\boldsymbol{D} \in \mathbb{R}^{n \times K}$. n is the number of rows, which is the product of the number of functions and attributes. Then we could train the weight of dictionary $\boldsymbol{w}$ instead of training $\Delta$ or $l$ directly. $\boldsymbol{w} \in \mathbb{R}^{n}$. n is the dimension of hyperparameter should be trained. High dimension will cause the problem of hypergradient estimation and bring instability and convergence issues. Normally we will use $n < K$. $\boldsymbol{\Delta} = \boldsymbol{w}_{\boldsymbol{\Delta}}^{\top}\mathbb{F}(\mathbb{A})$ and $\boldsymbol{\
% l} = \boldsymbol{w}_{\boldsymbol{l}}^{\top}\mathbb{F}(\mathbb{A})$. 

% For attributes $\mathbb{A}$, we use frequency ($\mathbb{A}_{\text{freq}}$) inspired by \cite{ye2020identifying} and \cite{menon2020long}, difficulty ($\mathbb{A}_{\text{diff}}$) which is related to the class error, the norms of the classifier weights ($\mathbb{A}_{\text{norm}}$) inspired by \cite{kang2019decoupling}; For function $\mathbb{F}$, we use polynomial inspired by \cite{ye2020identifying} and log function inspired by \cite{menon2020long}.

% \iffalse
% \subsubsection*{challenge of bilevel optimazation}
% \textbf{warm-up:} In bilevel training, the warm-up phase is essential to guarantee that the IFT assumption $\frac{\partial \mathcal{L}_{\text {train }}\left(\boldsymbol{\theta}^{\star}, \boldsymbol{\alpha}^{\star}\right)}{\partial \boldsymbol{\theta}}=0$ is approximately satisfied. But as shown in Table\ref{table:warmup_result}, warm-up in a more balanced way could get better result. If search phase start with biased model parameters, then it's hard to escape from it and will influence the final result. So we have reason to believe that if we could reduce warm-up training epochs and start search phase with more balanced initial model parameters, we could improve the result and improve efficiency. We proposed dictionary to train hyperparameters with restricted degrees of freedom and it make it possible for us to train with only 5 epochs warming up and achieve a good result.\\
% \fi


% \iffalse
% \textbf{Stability:}From the evolution of hyperparameters Figure\ref{fig:stable}, we could find that there are some sudden gap during the training and the sort of the hyperparameters doesn't always follow the sort that a larger class need a larger value. After adding dictionary, the attributs could be used as pilots which could reduce the number of parameter and strict the sort of hyperarameters.
% \fi

% \begin{wrapfigure}{r}{0.80\textwidth}
% \begin{subfigure}[t]{0.38\textwidth}
% 		\begin{tikzpicture}
% 			\node at (0,0) {\includegraphics[scale=0.48]{./figs/fig_dyly_AB.pdf}};
% 			\node at (-4,0) [scale=0.8,rotate=90]{Hyper-parameter value};
% 			\node at (0,-3) [scale=0.8]{Epoch};
% 		\end{tikzpicture}\vspace{-8pt}\caption{Autobalance without dictionary}\label{fig:stable_aut}
% 	\end{subfigure}~
% 	\begin{subfigure}{.2\linewidth}
% 		\begin{tikzpicture}
% 			\node at (0,0) {\includegraphics[scale=0.48]{./figs/fig_dyly_dic.pdf}};
% 			\node at (-4,0) [scale=0.8,rotate=90]{Hyper-parameter value};
% 			\node at (0,-3) [scale=0.8]{Epoch};
% 		\end{tikzpicture}\vspace{-8pt}\caption{Autobalance with dictionary}\label{fig:stable_dic}
% 	\end{subfigure}\caption{\mli{Xuechen: Larger legend and larger ticks.} Evolution of loss function parameters $l$, $\Delta$ over epochs for CIFAR10-LT where solid curves and dashed curves corresponds to $\Delta$ and $l$ respectively. After adding dictionary, the training is more stable.}\label{fig:stable}\vspace{-20pt}
% \end{wrapfigure}
%\input{automl/sec/stable_img}
% \begin{figure}
% \begin{subfigure}{0.32in}
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.155]{\includegraphics{./figs/fig_dyly_AB.pdf}};
% 		\node at (-1.7 ,0) [scale=0.6,rotate=90] {Hyper-parameter value};
% 		\node at (0.1,-1.3) [scale=0.6] {Epoch};
% 	\end{tikzpicture}\vspace{-8pt}\caption{Autobalance without dictionary}\label{fig:stable_aut}
% \end{subfigure}~
% \begin{subfigure}{0.32in}
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.16]{\includegraphics{./figs/fig_dyly_dic.pdf}};
% 		\node at (-1.75,0) [scale=0.6,rotate=90] {Hyper-parameter value};
% 		\node at (0.1,-1.3) [scale=0.6] {Epoch};
% 	\end{tikzpicture}\vspace{-8pt}\caption{Autobalance with dictionary}\label{fig:stable_dic}
% \end{subfigure}
% \caption{\small{\mli{Xuechen: Larger legend and larger ticks.} Evolution of loss function parameters $l$, $\Delta$ over epochs for CIFAR10-LT where solid curves and dashed curves corresponds to $\Delta$ and $l$ respectively. After adding dictionary, the training is more stable.}}\vspace{-10pt}%\eqref{deo eq} 
% \label{fig:stable}
% \end{figure}
%Based on previous observation, we proposed the dictionary strategy which is adding attributes such as class frequency to help bilevel training.
% \iffalse
% \subsubsection{attributes}
% \textbf{Why attributes} Using attributes could help to reduce the number of parameters. In post-hoc, a large amount of parameters could cause problem as we only have a few samples. In bilevel it also cause instability. Attributes \\

% \textbf{Is frequency all we need?} We try to fix the influence depend on classes. There are several papers modified training loss based on the label frequencies and achieve promising result. But class frequency is not the only reason for feature deviation in the test data. Bias is not always easy to quantify. The reason might be complex and be the cross term of several factors. So we designed the dictionary strategy which could help us make the use of known information but not be restricted by those specific and simple conditions.\\
% \fi
\subsection{Class-specific Learning Strategies: Bilevel Optimization and Post-hoc optimization}\label{sec:imp_bilevel_posthoc}
\input{sec/tab_bilevel}
To instantiate $\name$ as a meta-strategy, we focus on two important class-specific optimization problems: loss function design via bilevel optimization and post-hoc logit adjustment. We describe them in this section and demonstrate that both methods outperform the state-of-the-art approaches. The figure in Appendix illustrates how CAP is implemented under bi-level optimization and post-hoc optimization in detail.

\noindent$\bullet$ \textbf{Strategy 1: Loss function design via bilevel optimization.} Inspired by \cite{li2021autobalance} and following our exposition in Section \ref{sec:attributes}, we formalize the meta-strategy optimization problem as \[\min_{\w_\lb,\w_\Deltab}\Lc_{\text{val}}(\w_\lb,\w_\Deltab,f) \quad \mathrm{ s.t. }\quad \min_{f}\Lc_{\text{train}}(\w_\lb,\w_\Deltab,f) \]
where $f$ is the model and $\Lc_{\text{val}}$, $\Lc_{\text{train}}$ are validation and training losses respectively. Our goal is finding \name parameters $\w_\lb,\w_\Deltab$ that minimize the validation loss which is the target fairness objective.  Following the implementation of \cite{li2021autobalance}, we split the training data to 80\% training and 20\% validation to optimize $\Lc_{\text{train}}$ and $\Lc_{\text{val}}$. The optimization process is split to two phases: the search phase that finds \name parameters $\w_{\lb},\w_{\Deltab}$ and the retraining phase that uses the outcome of search and entire training data to retrain the model. We note that, during initial search phase, \cite{li2021autobalance} employs a long \textit{warm-up} phase where they only train $f$ while fixing $\w_\lb,\w_\Deltab$ to achieve better stability. In contrast, we find that \name either needs very short warm-up or no warm-up at all pointing to its inherent stability.
%, we also use the warm-up in our experiments but present more experiments in supplementary material showing that warm-up is often not necessary in our $\name$ approach.

\noindent$\bullet$ \textbf{Strategy 2: Post-hoc optimization.} In \cite{menon2020long,feldman2015certifying,hardt2016equality}, the author displays that the post-hoc logit adjustment can efficiently address the bias when training with imbalanced datasets. Formally, given a model $f$, a post-hoc function $g: \mathbb{R}^K\rightarrow \mathbb{R}^K$ adjusts the output of $f$ to minimize the fairness objective. Thus the final model of post-hoc optimization is $g\circ f(\x)$. %We remark that different from bilevel optimization, $g$ is optimized from test data following the same setup as \cite{menon2020long,feldman2015certifying,hardt2016equality}.



% In autobalace \cite{li2021autobalance} and VS loss \cite{kini2021label}, the loss is designed as 
% $\ell(y, f(\boldsymbol{x}))=w_{y} \log \left(1+\sum_{k \neq y} e^{l_{k}-l_{y}} \cdot e^{\Delta_{k} f_{k}(\boldsymbol{x})-\Delta_{y} f_{y}(\boldsymbol{x})}\right)$. We use smaller hyperparameters for minority classes to provide larger margin. It should be opposite when doing logits adjustment for post-hoc. Larger parameters should be used to increase the logits value of minority classes. Then the post-hoc model $g$ could be defined as $\boldsymbol{\alpha}$ for $\hat{f}_{y}=g \circ f_{y}\left(\boldsymbol{x}\right) = \frac{f_{y}\left(\boldsymbol{x}\right)}{\sigma\left(\Delta_{y}\right)}-l_{y}$\\
% \iffalse
% \textbf{post-hoc with dictionary}
% While training post-hoc, we still training $\boldsymbol{w} = [\boldsymbol{w}_{\boldsymbol{\Delta}},\boldsymbol{w}_{\boldsymbol{l}}]$ for each attributes' function $\mathbb{F}(\mathbb{A})$  instead of training $\boldsymbol{\Delta}$ and $\boldsymbol{l}$ freely. Surprising, we found that we could use post-hoc correction result directly on loss adjustment and still get a better result. \\

% \subsection{Transferring Post-hoc to loss design }
% \subsection{Initial with self-sup backbone}
% \fi
















==> sec/numeric.tex <==
\section{Experimental Evaluations}
\subsection{bilevel}
For bilevel training, we train $w_{dy}$ and $w_{ly}$ instead of training dy and ly directly. 
$dy = w_{dy}^\top f(\text{attributes})$ and $ly = w_{ly}^\top f(\text{attributes})$
\subsection{post-hoc}
We use a small subset of test dataset to train the post-hoc. For Cifar-10, if we have more than 50 samples in each class, the post-hoc model can be well trained. By adding attributes which is correlated to difficulty, we could improve the worse case accuracy without hurting balanced accuracy. This always happen at the end of the training. The result for balanced Cifar-10 also verify this conclusion. (balanced acc: 92.9 to 93.06, worst class accuracy: 83.4 to 85.5)
\subsection{Imbalance}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table}[]
% \begin{tabular}{|l|ll|ll|}
% \hline
% \multirow{2}{*}{} & \multicolumn{2}{l|}{Cifar-10}           & \multicolumn{2}{l|}{Cifar-100}          \\ \cline{2-5} 
%                   & \multicolumn{1}{l|}{post-hoc} & retrain & \multicolumn{1}{l|}{post-hoc} & retrain \\ \hline
% tau=1             & \multicolumn{1}{l|}{22.71}    & 23.06   & \multicolumn{1}{l|}{59.09}    & 58.39   \\ \hline
% Train: ly         & \multicolumn{1}{l|}{20.76}    & 20.48   & \multicolumn{1}{l|}{57.67}    & 57.07   \\ \hline
% dy*               & \multicolumn{1}{l|}{22.64}    & 20.93   & \multicolumn{1}{l|}{58.49}    & 57.06   \\ \hline
% Train:lydy        & \multicolumn{1}{l|}{21.64}    & 22.04   & \multicolumn{1}{l|}{57.68}    & 58.59   \\ \hline
% Grid search:lydy  & \multicolumn{1}{l|}{22.42}    & 23.46   & \multicolumn{1}{l|}{57.97}    & 63.96   \\ \hline
% \end{tabular}
% \end{table}
% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
%       & Cifar-10     &               \\ \hline
%       & post-hoc     & retrain       \\ \hline
% CE     & 12.95(11.39) & /             \\ \hline
% Dic:ly & 12.23(10.98) & 12.05(10.94)  \\ \hline
% Dic:dy & 12.74(11.02) & 12.72((10.37) \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%             & Cifar-10    &             & Cifar-100    &              \\ \hline
%             & post-hoc    & retrain     & post-hoc     & retrain      \\ \hline
% CE          & 14.35(8.35) & /           & 39.39(13.90) & /            \\ \hline
% Dic:ly      & 14.12(6.49) & 13.91(8.11) & 39.64(12.68) & 38.78(13.82) \\ \hline
% Dic:dy      & 14.18(7.77) & 12.87(7.48) & 39.58(13.64) & 38.81(13.68) \\ \hline
% Dic:lydy    & 14.13(7.53) & 13.93(7.94) & 39.65(13.49) & 38.76(13.77) \\ \hline
% \end{tabular}
% \end{table}
% \begin{table*}[t]
%     \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%                   & Cifar-10          &                & Cifar-100         &                \\ \hline
%                   & Balanced accuracy & Worst accuracy & Balanced accuracy & Worst accuracy \\ \hline
% CE                & 67.67             & 64.6           & 35.58             & 0              \\ \hline
% No attributes     & 76.58             & 61.8           & 36.82             & 0              \\ \hline
% Dic:freq          & 76.70             & 65.1           & 38.90             & 0.03           \\ \hline
% Dic:difficulty    & 76.07             & 67.1           & 37.87             & 0.03           \\ \hline
% Dic:norm          & 76.54             & 62.4           & 38.42             & 0.03           \\ \hline
% Dic:all (6 para)  & 76.59             & 65.33          & 38.83             & 0.03           \\ \hline
% Dic:all (10 para) & 76.68             & 65.55          & 38.95             & 0.03           \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
%     \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \#sample per class & LA          & Attributes: Freq & Attributes: all \\ \hline
% 1000               & 78.74(63.1) & 79.32(65.3)      & 79.28(67.4)     \\ \hline
% 100                & 78.67(63.0) & 79.24(65.4)      & 79.18(67.9)     \\ \hline
% 50                 & 78.66(63.0) & 79.06(64.6)      & 79.3(66.5)      \\ \hline
% 10                 & 78.4(62.4)  & 78.79(63.8)      & 78.75(63.8)     \\ \hline
% 1                  & 71.58(46.7) & 71.85(48.9)      & 71.68(49.5)     \\ \hline
% \end{tabular}
% \end{table*}

% \iffalse
% \begin{table*}[t]
%     \centering
% \begin{tabular}{|l|l|l|l||}
% \hline
% \#sample per class & LA          & No dic & Attributes: Freq & Attributes: all \\ \hline
% 1000               & 78.74(63.1) & & 79.32(65.3)      & 79.28(67.4)     \\ \hline
% 100                & 78.67(63.0) & 78.42(67.6)&79.24(65.4)      & 79.18(67.9)     \\ \hline
% 50                 & 78.66(63.0) & &79.06(64.6)      & 79.3(66.5)      \\ \hline
% 10                 & 78.4(62.4)  & &78.79(63.8)      & 78.75(63.8)     \\ \hline
% 1                  & 71.58(46.7) & &71.85(48.9)      & 71.68(49.5)     \\ \hline
% \end{tabular}
% \end{table*}
% \fi

% \subsection{Group}
% \iffalse
% \begin{table}[t]
%     \centering
% \begin{tabular}{|l|l|}
% \hline
%           & EMnist \\ \hline
% CE        & 87.6   \\ \hline
% No dic    & 89.3   \\ \hline
% Dic: diff & 90.6   \\ \hline
% \end{tabular}
% \end{table}
% \fi
% \subsection{Noisy label}
% We validate our method on balanced and imbalanced CIFAR-10 and CIFAR-100. We use symmetric label noise which is generated by randomly replacing the labels for a percentage of the training data with all possible labels instead of the previous label. The percentage of each class is random value in the range (0,0.3). The probability that the new label is generated corresponds to class frequency.
% \begin{table}[]
% \begin{tabular}{|ll|l|l|l|l|}
% \hline
% \multicolumn{2}{|l|}{\multirow{2}{*}{}}                      & Cifar-10     &               & Cifar-100    &              \\ \cline{3-6} 
% \multicolumn{2}{|l|}{}                                       & post-hoc     & retrain       & post-hoc     & retrain      \\ \hline
% \multicolumn{2}{|l|}{CE}                                     & 42.88(22.65) & /             & 72.18(22.88) & /            \\ \hline
% \multicolumn{1}{|l|}{Dic:ly}                    & freq       & 37.21(10.73) & 35.75(12.30)  & 70.25(17.67) & 68.84(18.24) \\ \hline
% \multicolumn{1}{|l|}{}                          & error      & 36.36(7.98)  & 34.81(6.48)   & 71.42(16.5)  & 70.69(20.19) \\ \hline
% \multicolumn{1}{|l|}{}                          & freq+error & 36.19(8.6)   & 35.11(8.94)   & 70.55(17.12) & 70.62(15.69) \\ \hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{Dic:dy}}   & freq       & 36.97(17.65) & 37.44((16.38) & 70.85(20.08) & 69.36(16.81) \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                          & error      & 39.35(18.52) & 38.78(18.23)  & 71.05(20.29) & 70.82(19.08) \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                          & freq+error & 36.63(17.63) & 35.72(14.78)  & 71.26(19.81) & 70.30(14.86) \\ \hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{Dic:dyly}} & freq       & 37.25(11.3)  & 35.15(11.95)  & 70.19(18.81) & 71.07(15.06) \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                          & error      & 36.7(6.62)   & 38.48(13.71)  & 71.35(18.26) & 71.65(18.46) \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                          & freq+error & 35.91(7.63)  & 36.36(11.70)  & 70.81(17.95) & 71.66(13.28) \\ \hline
% \multicolumn{2}{|l|}{No dic: ly}                             & 38.14(16.79) & 36.04(14.42)  & 70.26(19.31) & 71.21(18.30) \\ \hline
% \multicolumn{2}{|l|}{No dic: dy}                             & 39.07(21.72) & 37.91(17.21)  & 70.66(22.46) & 69.51(20.80) \\ \hline
% \multicolumn{2}{|l|}{No dic: lydy}                           & 38.66(19.97) & 37.12(16.15)  & 70.66(22.46) & 70.50(20.81) \\ \hline
% \end{tabular}
% \end{table}
% \subsection{Self-sup}
% \begin{table}[t]
%     \centering
% \begin{tabular}{|l|l|l|}
% \hline
%             & Cifar-10 & Cifar-100 \\ \hline
% weighted CE & 70.90    & 38.52     \\ \hline
% tau=1       & 70.87    & 38.59     \\ \hline
% post-hoc    & 71.20    & 38.71     \\ \hline
% \end{tabular}
% \end{table}


==> sec/setup.tex <==
%!TEX root = ../automl.tex
\vspace{-4pt}
\section{Problem Setup}

This paper investigates the advantages of utilizing attribute-based personalized training approaches for addressing heterogeneous classes in the context of class imbalance, label noise, and fairness objective problems. We begin by presenting the general framework, followed by an examination of specific fairness issues, which encompass both distributional and objective heterogeneities.
Consider a multi-class classification problem for a dataset $ (\x_i,y_i)^{N}_{i=1}$ sampled i.i.d from a distribution with input space $\Xc$ and $K$ classes. Let $[K]$ denote the set $\{1..K\}$ and for the training sample $(\x,y)$, $\x \in \Xc$ is the input and $y\in [K]$ is the output. $f: \Xc\rightarrow \mathbb{R}^K$ represents the model and $\lgt$ is the output logits.  $\hat{y}_{f(\x)}=\text{arg max}_{k\in [K]} \lgt_k$ is the predicted label of the model $f(\x)$. We also denote $K\times K$ identity matrix by $\bm{I}_K$. Moreover, in the post-hoc setup, a logit adjustment function $g: \mathbb{R}^K\rightarrow \mathbb{R}^K$ is employed to modify the logits, resulting in adjusted logits $\hat{\lgt}= g(\lgt)$. 

Our goal is to train a model that minimizes a specific classification error metric. The class-conditional errors are defined over the data distribution as 
$
\err_{k}=\mathbb{P}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=k\right]
$. The standard classification error is denoted by $\serr=\mathbb{P}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\right]$. In situations with label imbalance, $\serr$ is dominated by the majority classes. To this end, balanced classification error $\berr=\frac{1}{K} \sum_{k=1}^{K}\kerr$ is widely employed as a fairness metric. We will later introduce other objectives that aim to achieve different fairness goals. A complete list of the objectives we examine can be found in Appendix. 
%\ref{app:syms}.

% Additionally, we introduce objectives that aims to achieve different fairness goal such as the balanced misclassification error $\berr=(1 / K) \sum_{k=1}^{K}\mathcal{E}_{\mathrm{k}}$, 
%  errors of quantile classes $\quan = \mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]$($\mathrm{K}_{a}$ are the quantile classes determined by level $\mathrm{a}$), 
%  Standard deviation of class-conditional errors $\dev = \text{std}(\err)$,
%  Conditional value of errors at level $\cv = \mathbb{E}\left(\mathcal{E}_{k}\mid \mathcal{E}_{k}>\quan\right)$ and Weighted misclassification error $\werr=(1 / K) \sum_{k=1}^{K}w\mathcal{E}_{\mathrm{k}}$.
 
% \[
% \text{Balanced misclassification error:}~
% \mathcal{E}_{\mathrm{bal}}(f)=(1 / K) \sum_{k=1}^{K} \mathcal{E}_{\mathrm{k}}(f).
% \]
% \[
% \quad\text{Standard deviation of class-conditional errors:}~\mathcal{S}= \sqrt{(1 / K) \sum_{k=1}^{K}\left[(\mathcal{E}_{k}-\mathcal{E}_{\mathrm{bal}})^{2}\right]}.
% \]
% \[
% \quad\text{Errors of quantile classes at level $a$, measures the selected classes behaviour:}~ \mathcal{Q}_{a}(\mathcal{E}) = \mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]\text{, } \mathrm{K}_{a} \text{are the quantile classes determined by level } \mathrm{a}
% \]
% \[
% \quad\text{Conditional value of errors at level $a$,measures the tail behaviour:}~ \mathcal{C}_{a}(\mathcal{E}) = \mathbb{E}\left(\mathcal{E}_{k}\mid \mathcal{E}_{k}>\mathcal{Q}_{a}(\mathcal{E})\right)
% \]
% \[
% \quad\text{Weighted misclassification error:}~ \werr=(1 / K) \sum_{k=1}^{K}w\mathcal{E}_{\mathrm{k}}
% \]
% Naturally, the balanced misclassification error is defined as $
% \mathcal{E}_{\mathrm{bal}}(f)=(1 / K) \sum_{k=1}^{K} \mathcal{E}_{\mathrm{k}}(f)
% $ and the standard deviation of error among each classes is defined as $
% \mathcal{S}(f)= \sqrt{(1 / K) \sum_{k=1}^{K}\left[(\mathcal{E}_{k}(f)-\mathcal{E}_{\mathrm{bal}}(f))^{2}\right]}$. Throughout the paper, we use the balanced misclassification error for evaluation.
% \xuechen{per class error and entire error, should be use different symbol?}
%\xuechen{Question:1.header,backbone,predictor. Which one is defined as f? 2.dictionary and distribution. $\mathcal{D}$ and $\Dic$. Similar}

% \textbf{risks}
% \[
% \text{Balanced risk:}~\aci{bal}{f}=\frac{1}{K}\sum_{k=1}^K\aci{k}{f}\quad \text{and} \quad \text{Class-conditional risk:}~\aci{k}{f}=\E_{\Dc_k}[\ell(y,\yh_f(\x))].
% \]
% \xuechen{Risks of quantile classes: $\mathcal{Q}_{a}(\mathcal{E}(f)) = \mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]$, $\mathrm{K}_{a}$ are the quantile classes determined by level a}\\ 
% \xuechen{Conditional value: $\mathcal{C}_{a}(\mathcal{E}(f)) = \mathbb{E}\left(\mathcal{E}_{k}(f)\mid \mathcal{E}_{k}(f)>\mathcal{Q}_{a}(\mathcal{E}(f))\right)$ }\\
% \xuechen{Aggregation: We combine different objectives via an aggregator. }
% \iffalse
% \textbf{Data:}
% Suppose we have a dataset $\Sc = (\x_i,y_i)^{n}_{i=1}$ sampled i.i.d from $\Dc$ with input space $\Xc$ and $K$ classes. For a training sample $(\x,y)$, $\x \in \Xc$ is the input and $y\in [k]$ is the output label where $[K]$ denote the set $\{1..K\}$. The frequency of the k’th class is defined as $
% \boldsymbol{\pi}_{k}=\mathbb{P}_{(\boldsymbol{x}, y) \sim \mathcal{D}}(y=k)
% $.Label/class-imbalance occurs when the class frequencies differ substantially.\\

% \textbf{Evaluation metrics:} The standard classification error is 
% $\mathcal{E}(f)=\mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\right]
% $. The class-conditional risks are defined as 
% $
% \mathcal{E}_{k}(f)=\mathbb{P}_{\mathcal{D}}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=k\right]
% $. The balanced error is the average of the error of each classes, $
% \mathcal{E}_{\mathrm{bal}}(f)=(1 / K) \sum_{k=1}^{K} \mathcal{E}_{\mathrm{k}}(f)
% $. The fairness is evaluated by computing the standard deviation of error among each classes $
% \mathcal{S}(f)= \sqrt{(1 / K) \sum_{k=1}^{K}\left[(\mathcal{E}_{k}(f)-\mathcal{E}_{\mathrm{bal}}(f))^{2}\right]} 
% $. 
% \fi
%\mli{Should we put specific loss function here?}




 
 

==> sec/stable_img.tex <==
\begin{figure}
\centering
\begin{subfigure}{2.32in}
	\begin{tikzpicture}
		\node at (0,0) [scale=0.255]{\includegraphics{./figs/fig_dyly_AB.pdf}};
		\node at (-2.5 ,0) [scale=0.6,rotate=90] {Hyper-parameter value};
		\node at (0.1,-1.3) [scale=0.6] {Epoch};
	\end{tikzpicture}\vspace{-8pt}\caption{without dictionary}\label{fig:stable_aut}
\end{subfigure}~
\begin{subfigure}{2.32in}
	\begin{tikzpicture}
		\node at (0,0) [scale=0.26]{\includegraphics{./figs/fig_dyly_dic.pdf}};
		\node at (-2.5,0) [scale=0.6,rotate=90] {Hyper-parameter value};
		\node at (0.1,-1.3) [scale=0.6] {Epoch};
	\end{tikzpicture}\vspace{-8pt}\caption{with dictionary}\label{fig:stable_dic}
\end{subfigure}
\caption{\small{\mli{Xuechen: Larger legend and larger ticks.} Evolution of loss function parameters $l$, $\Delta$ over epochs for CIFAR10-LT where solid curves and dashed curves corresponds to $\Delta$ and $l$ respectively. After adding dictionary, the training is more stable.}}\vspace{-10pt}%\eqref{deo eq} 
\label{fig:stable}
\end{figure}

==> sec/tab_attributes.tex <==
\begin{wrapfigure}{t}{.3\linewidth}\vspace{-8pt}
		\begin{minipage}{\linewidth}
		%\begin{table}
	\begin{center}\resizebox{\textwidth}{!}{
			\begin{tabular}{lll}
				\toprule
                                     & $\berr$&$\dev$               \\
\toprule                              
$\nodic$                           & 40.04&31.69  \\ 


 $\att_{\text{freq}}$        & 39.84&26.68 \\
 $\att_{\text{diff}}$       & 40.78&14.31  \\
$\att_{\text{freq}}$ \& $\att_{\text{diff}}$ & 38.79&20.05  \\ 


\bottomrule
		\end{tabular}}\caption{\xuechen{Dictionary attributes:setting B, lt dataset with noisy label, bilevel}Evaluations of balanced error and standard deviation among each classes on long-tailed data with noisy label.\xuechen{change to noisy ratio result?}}\label{table:attributes}\vspace{-2pt}
	\end{center}
		%\end{table}
	\end{minipage}
\end{wrapfigure}

==> sec/tab_attributes_definition.tex <==
\begin{wrapfigure}{t}{1\linewidth}\vspace{-6pt} 
		\begin{minipage}{\linewidth}
		%\begin{table}
	\begin{center}\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\toprule
 Attributes            & Definition & Cases \\
\midrule
 $\att_{\text{freq}}$         & class frequency & Designed for imbalance datasets.\\
 $\att_{\text{diff}}$         & class-conditional risks & \makecell[l]{Overweight bad-performance classes. \\Could be used without knowing the reason of imbalance. \\ Performs good for target classes related objectives.}\\
 $\att_{\text{weights}}$      & new weights for target distribution & Designed for distribution shift.\\
 $\att_{\text{noisy}}$ & noise ratio & Designed for datasets with noisy label.\\
 $\att_{\text{norm}}$ &  norm of the weight vectors of the last fully-connected layer & Label-distribution-aware value. Could be used without knowing class frequency. \\
  ... &   & \\
\bottomrule
		\end{tabular}}\caption{Definition of attributes and using cases}\label{table:attributes_definition}\vspace{-6pt}
	\end{center}
		%\end{table}
	\end{minipage}
\end{wrapfigure}

==> sec/tab_attributes_lt.tex <==
% \begin{wrapfigure}{t}{.4\linewidth}\vspace{-8pt}
% 		\begin{minipage}{\linewidth}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lllll}
% 				\toprule
% \multicolumn{1}{l}{\multirow{2}{*}{}} & \multicolumn{2}{l}{Cifar100-LT} & \multicolumn{2}{l}{ImageNet-LT} \\
% \toprule
% \multicolumn{1}{l}{}                  & $\berr$&$\dev$            & $\berr$&$\dev$          \\
% \midrule
%  $\nodic$     &  56.70              &    20.13         &  50.91              &   26.06             \\
%  $\att_{\text{freq}}$     &  56.64              &    19.10         &  50.88              &   24.38             \\
%                           $\att_{\text{diff}}$      &  58.27              &   17.62             &     53.04  &           21.02             \\
%                           $\att_{\text{freq}}$+$\att_{\text{diff}}$&   56.38             &     18.53           &    49.32            &  21.94              \\
% \bottomrule
% 		\end{tabular}}\caption{Dictionary attributes:setting A. Evaluations of balanced error and standard deviation among each classes on long-tailed datasets.}\label{table:attributes_lt}\vspace{-2pt}
% 	\end{center}
% 	\end{minipage}
% \end{wrapfigure}

\begin{wrapfigure}{t}{1\linewidth}\vspace{-8pt}
		\begin{minipage}{\linewidth}
	\begin{center}\resizebox{\textwidth}{!}{
			\begin{tabular}{lllllll}
				\toprule
\multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{2}{l}{Cifar100-LT} & \multicolumn{2}{l}{ImageNet-LT} & \multicolumn{2}{l}{Cifar10-LT w. noisy}\\
\toprule
\multicolumn{1}{l}{}                  & $\berr$&$\dev$ & $\berr$&$\dev$            & $\berr$&$\dev$          \\
\midrule
 $\nodic$     &  56.70              &    20.13         &  50.91              &   26.06      &40.04 &   31.69    \\
 $\att_{\text{freq}}$     &  56.64              &    19.10         &  50.88              &   24.38       & 39.84&  26.68    \\
                           $\att_{\text{diff}}$     &  58.27              &   17.62             &     53.04  &           21.02         & 40.78&  14.31   \\
                           $\att_{\text{freq}}$+$\att_{\text{diff}}$  &   56.38             &     18.53           &    49.32            &  21.94            & 38.79& 20.05 \\
\bottomrule
		\end{tabular}}\caption{Dictionary attributes:setting A. Evaluations of balanced error and standard deviation among each classes on long-tailed datasets.}\label{table:attributes_lt}\vspace{-2pt}
	\end{center}
	\end{minipage}
\end{wrapfigure}

==> sec/tab_attributes_lt_old.tex <==
\begin{wrapfigure}{t}{.4\linewidth}\vspace{-8pt}
		\begin{minipage}{\linewidth}
		%\begin{table}
	\begin{center}\resizebox{\textwidth}{!}{
			\begin{tabular}{lllll}
				\toprule
\multicolumn{1}{l}{\multirow{2}{*}{}} & \multicolumn{2}{l}{Cifar100-LT} & \multicolumn{2}{l}{ImageNet-LT} \\
\toprule
\multicolumn{1}{l}{}                  & $\mathcal{E}_{\mathrm{\text{bal}}}(f)$&$\mathcal{S}(f)$            & $\mathcal{E}_{\mathrm{\text{bal}}}(f)$&$\mathcal{S}(f)$          \\
\midrule
 $\att_{\text{freq}}$     &  57.70              &    19.17         &  52.04              &   25.44             \\
                           $\att_{\text{diff}}$      &  59.31              &   18.00             &     53.55  &           23.06             \\
                           $\att_{\text{freq}}$+$\att_{\text{diff}}$&   57.68             &     18.67           &    51.50            &  23.93              \\
% \midrule
% \multirow{3}{*}{Bilevel}  & freq      &                &            &    &                &           &     \\\cline{3-8} 
%                           & diff      &                &            &    &                &              &  \\\cline{3-8} 
%                           & freq+diff &                &            &    &                &            &   \\
\bottomrule
		\end{tabular}}\caption{Evaluations of balanced error and standard deviation 
among each classes on long-tailed.\xuechen{Adding quantile? difficulty helps worst classes; compare more attributes? }}\label{table:attributes_lt}\vspace{-2pt}
	\end{center}
		%\end{table}
	\end{minipage}
\end{wrapfigure}

==> sec/tab_attributes_objective.tex <==

% \begin{wrapfigure}{t}{1\linewidth}\vspace{-8pt}
% 		\begin{minipage}{\linewidth}
% 		%\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lllllllllll}
% 				\toprule
% \multicolumn{1}{l}{} & \multicolumn{5}{l}{Cifar100-LT} & \multicolumn{5}{l}{ImageNet-LT} \\
% \toprule
% \multicolumn{1}{l}{}                  & $\bacc$            & $\wacc$  & $\std$ & $\cv$ &$\quan$  & $\bacc$            & $\wacc$  & $\std$ & $\cv$ &$\quan$    \\
% \midrule
%   $\nodic$     &    9.84          &  8.30  & 4.89  & 10.21  & 11.23   &  7.63            &    &   &   &           \\
%  $\att_{\text{freq}}$     &     10.99         &  9.01  & 11.56  & 8.20  & 7.57   &   8.77           &    &   &   &           \\
%  $\att_{\text{other}}$    &      9.38       & 9.91   &  12.77 & 9.85  & 11.94   &    7.26          &    &   &   &            \\
%  $\att_{\text{freq}}$ \& $\att_{\text{other}}$&   11.21     &  11.32            &  12.78  & 12.02  & 12.18  & 9.31   &             &    &   &               \\

% \bottomrule
% 		\end{tabular}}\caption{Evaluations of different objective. Post-hoc improvement\xuechen{new }}\label{table:attributes_objective}\vspace{-2pt}
% 	\end{center}
% 		%\end{table}
% 	\end{minipage}
% \end{wrapfigure}

% \begin{wrapfigure}{t}{0.6\linewidth}\vspace{-8pt}
% 		\begin{minipage}{\linewidth}
% 		%\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lllll}
% 				\toprule
% %\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
% %\toprule
% \multicolumn{1}{l}{}                  & $\berr$              & $\dev$ & $\cv$ &$\quan$  \\
% \midrule
% $\pretrain$&        62.74        & 38.96  & 96.95  &  95.15  \\
%   $\nodic$     &    -9.84            & -4.89  & -10.21  & -11.23   \\
%  $\att_{\text{freq}}$     &     -10.99           & -11.56  & -8.20  & -7.57   \\
%  $\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
%  $\att_{\text{freq}}$ \& $\att_{\text{diff}}$&   -11.21                &  -12.78  & -12.02  & -12.18  \\

% \bottomrule
% 		\end{tabular}}\caption{\xuechen{Dictionary attributes:setting C, lt dataset, post-hoc, different objective}Evaluations of different objective. Post-hoc improvement. \xuechen{Question: Should we put weighted acc here? Not Attributes:difficulty}}\label{table:attributes_objective}\vspace{-2pt}
% 	\end{center}
% 		%\end{table}
% 	\end{minipage}
% \end{wrapfigure}

% \begin{wrapfigure}{t}{0.4\linewidth}\vspace{-8pt}
% 		\begin{minipage}{\linewidth}
% 		%\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{

% \begin{tabular}{ll}
% \toprule
%              & Error \\
% \midrule
% $\pretrain$    & 62.53 \\
% $\nodic$        & -2.30 \\
%  $\att_{\text{freq}}$         & -3.79 \\
%  $\att_{\text{weights}}$      & -1.74 \\
%  $\att_{\text{freq}}$+ $\att_{\text{weights}}$ & -5.42\\

% \bottomrule
% 		\end{tabular}}\caption{weighted error(random weights)}\label{table:attributes_objective}\vspace{-2pt}
% 	\end{center}
% 		%\end{table}
% 	\end{minipage}
% \end{wrapfigure}

\begin{wrapfigure}{t}{1\linewidth}\vspace{-8pt}
		\begin{minipage}{\linewidth}
		%\begin{table}
	\begin{center}\resizebox{\textwidth}{!}{
			\begin{tabular}{llllll}
				\toprule
%\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
%\toprule
\multicolumn{1}{l}{}                  & $\berr$              & $\dev$ & $\cv$ &$\quan$ &$\werr$ \\
\midrule
$\pretrain$&        61.94        & 38.96  & 96.95  &  95.15 &62.53 \\
  $\nodic$     &    -1.62            & -4.89  & -10.21  & -11.23 &-2.30  \\
  LA  &       -3.73        & -9.53  & -10.21  & -11.23 &  / \\
 Single Attributes     &    -4.23($\att_{\text{freq}}$)           & -12.77($\att_{\text{diff}}$)  & -9.85($\att_{\text{diff}}$)  & -11.94($\att_{\text{diff}}$) & -3.79($\att_{\text{freq}}$)  \\
 %$\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
 Combining Attributes &  -4.36($\att_{\text{freq}}$\&$\att_{\text{diff}}$)              &  -12.78($\att_{\text{freq}}$\&$\att_{\text{diff}}$)  & -12.02($\att_{\text{freq}}$\&$\att_{\text{diff}}$)  & -12.18($\att_{\text{freq}}$\&$\att_{\text{diff}}$) & -5.42($\att_{\text{freq}}$\&$\att_{\text{weight}}$)\\

\bottomrule
		\end{tabular}}\caption{\xuechen{Dictionary attributes:setting C and Objective. lt dataset, post-hoc, different objective}Evaluations of different objective. Post-hoc improvement. }\label{table:attributes_objective}\vspace{-2pt}
	\end{center}
		%\end{table}
	\end{minipage}
\end{wrapfigure}




==> update/renew_obj_img.tex <==
\begin{figure}
\centering
%\hspace{-35pt}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{./figs/quantile_bar.pdf}};
		\node at (-2.3 ,0) [scale=0.8,rotate=90] {$\quan$ improvement};
		\node at (0,-1.9) [scale=0.8] {$a$};
	\end{tikzpicture}\vspace{-4pt}\caption{Errors of quantile classes\xuechen{working on}}\label{fig:obj_quan}
\end{subfigure}
\begin{subfigure}{1.8in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{./update/per_bar_1.pdf}};
		\node at (-2.5,0) [scale=0.8,rotate=90] {$\cv$ improvement};
		\node at (0,-1.9) [scale=0.8] {$a$};
	\end{tikzpicture}\vspace{-4pt}\caption{Conditional value of errors\xuechen{working on}}\label{fig:obj_cv}
\end{subfigure}
\begin{subfigure}{1.7in}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.29]{\includegraphics{./update/tradeoff_1.pdf}};
		\node at (-2.3,0) [scale=0.8,rotate=90] {Standard error ($\serr$)};
		\node at (0,-1.8) [scale=0.8] {Standard deviation ($\dev$)};
	\end{tikzpicture}\vspace{-4pt}\caption{Aggregation of errors}\label{fig:obj_agg}
\end{subfigure}
\hspace{35pt}
\caption{ Benefit of $\name$ for optimizing different Fairness Objectives. We compare among plain post-hoc, LA post-hoc and $\name_{\text{post-hoc}}$. (a):  Results of optimizing quantile class performance $\quan = \mathbb{P}\left[y \neq \hat{y}_{f}(\boldsymbol{x})\mid y=\mathrm{K}_{a}\right]$, where $\mathrm{K}_{a}$ denotes the class index with the worst $\lceil\mathrm{K}\times{a}\rceil$-th error. (b): Results of optimizing tail performance $\cv$. (c): Results of optimizing $\aggr= \lambda\cdot\serr+(1-\lambda)\cdot\dev$. The plot shows the trade-off between standard deviation of class-conditional errors $\dev$ and Standard misclassification error $\serr$ as $\lambda$ varies. See Sec.\ref{sec:objective} for detailed definition and discussions.}\vspace{-10pt}%\eqref{deo eq} 
\label{fig:obj}
\end{figure}
% \begin{wrapfigure}{t}{.4\linewidth}\vspace{-1pt}
% \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.32]{\includegraphics{./figs/tradeoff.pdf}};
% 		\node at (-2.5,0) [scale=1,rotate=90] {Standard error};
% 		\node at (0,-2) [scale=1] {Standard deviation};
% 	\end{tikzpicture}\vspace{-1pt}\caption{Objective setting C:  Results on $\aggr$. The plot shows the trade-off between standard deviation of class-conditional errors $\dev$ and Standard misclassification error $\serr$ as $a$ is varied.  The comparison is between original post-hoc, LA post-hoc and $\name_{\text{post-hoc}}$.\xuechen{1.name? 2. change to improvement, same as table for other 2 objectives}}\label{fig:stable_dic}
% \end{wrapfigure}

==> update/renew_result.tex <==
\section{New results with Standard Deviation}\label{app:new_result}
In this section, we provide the standard deviation of Table~\ref{table:dic}, \ref{table:posthoc}, \ref{table:attributes_lt}, \ref{table:attributes_objective} to Table~\ref{table:dic_supp}, \ref{table:posthoc_supp}, \ref{table:attributes_lt_supp}, \ref{table:attributes_objective_supp} respectively. 

% \begin{table}[]
% \centering
% \resizebox{0.8\textwidth}{!}{
% 			\begin{tabular}{lccc}
% 			\toprule
% 	Method		& CIFAR10-LT & CIFAR100-LT&ImageNet-LT\\
% 				\toprule
% 				 Cross entropy       & 30.45($\pm$0.49)           &  61.94($\pm$0.28) &55.52\\ 
% 				             Logit adjustment (LA)\cite{menon2020long}       & 21.29$\dagger$($\pm$0.43)            &  58.21$\dagger$($\pm$0.31) &52.46$\sharp$\\ 
% 			                 CDT\cite{ye2020identifying}      & 21.57$\dagger$($\pm$0.50)      & 58.38$\dagger$($\pm$0.33)  & 53.47$\sharp$\\                                                                                                                                         
% 			$\nodic_{\text{Bilevel}}$ 
% 			(AutoBalance \cite{li2021autobalance})   & 21.15$\sharp$ &56.70$\sharp$&50.91$\sharp$ \\ \cline{1-4}
% 			 $\name_{\text{Bilevel}}$: LA loss \cite{menon2020long}    & 21.82($\pm$0.32) &58.68($\pm$0.23)&52.39$\sharp$\\  
% 			 %$\name_{\text{AB}}$ $\gamma$ for CDT loss    & 22.67 &58.41&\\  
			
% 			  %$\name_{\text{Bilevel}}$ no init    & 20.41 &56.64&50.88\\ \cline{2-4}
% 			 %$\name_{\text{Bilevel}}$ LA init    & 20.22 &56.57&50.04\\  \cline{2-4}
% 			 $\name_{\text{Bilevel}}: \att$    & \textbf{20.22}($\pm$0.35) &\textbf{56.57}($\pm$0.26)&\textbf{50.04}\\  
% 			 %$\name_{\text{Bilevel}}$ without warm up & 20.16 &56.55&/\\ 
% 				\bottomrule %\vspace{10pt}
% 		\end{tabular}}\caption{Standard deviation results of Table~\ref{table:dic}. Balanced error on long-tailed data using loss function design via bilevel optimization. $\sharp$: best reported results taken from \cite{li2021autobalance}.$\dagger$: Reproduced results.}\label{table:dic_supp} \vspace{-20pt}
% \end{table}


\begin{table}[]
\centering
%\resizebox{\textwidth}{!}{
			\begin{tabular}{llllll}
			\toprule
			\multicolumn{2}{l}{}              & \multicolumn{2}{l}{CIFAR10-LT}& \multicolumn{2}{l}{CIFAR100-LT} \\
				\toprule
				\multicolumn{2}{l}{}              & search phase & retrain& search phase & retrain \\ 
		\toprule		
 \multicolumn{2}{l}{Post-hoc LA\cite{menon2020long} }  & 21.43($\pm$0.30)        & 22.34($\pm$0.34)&58.48($\pm$0.23)&57.65($\pm$0.25)   \\
\multicolumn{2}{l}{Post-hoc CDT\cite{ye2020identifying} }             & 23.58($\pm$0.37)        & 21.79($\pm$0.40) &58.60($\pm$0.26)&57.86($\pm$0.27)  \\ 
\midrule
    \multicolumn{1}{l}{\multirow{3}{*}{$\nodic_{\text{Post-hoc}}$}}   & $\boldsymbol{l}$                      & 20.90($\pm$0.28)        & 21.71($\pm$0.29) &57.98($\pm$0.22)&57.82($\pm$0.19)  \\ 
\multicolumn{1}{l}{}                                         & $\boldsymbol{\Delta}$                      & 23.74($\pm$0.34)        & 24.06($\pm$0.36) &58.61($\pm$0.29)&58.80($\pm$0.31)   \\  
\multicolumn{1}{l}{}                                         & $\boldsymbol{l}$\&$\boldsymbol{\Delta}$                  & 23.41($\pm$0.30)        & 23.38($\pm$0.33) &57.80($\pm$0.24)&58.57($\pm$0.23) \\                  

\midrule

\multicolumn{1}{l}{\multirow{3}{*}{$\name_{\text{Post-hoc}}$}}   & $\w_\lb$                      & 20.81 ($\pm$0.15)       & 20.65($\pm$0.36) &57.73($\pm$0.25)&57.15($\pm$0.30)  \\  
\multicolumn{1}{l}{}                                         & $\w_\Deltab$                      & 22.31($\pm$0.38)        & 21.06($\pm$0.43)  &58.07($\pm$0.32)&57.26($\pm$0.35) \\  

\multicolumn{1}{l}{}                                         & $\w_\lb$ \& $\w_\Deltab$                 & 20.87($\pm$0.38)        & 20.32($\pm$0.64) &57.63($\pm$0.26)&57.08($\pm$0.21)  \\ 
\bottomrule
		\end{tabular}\caption{Standard deviation results of Table~\ref{table:posthoc}. Balanced error on long-tailed data using post-hoc logits adjustment. The search phase results reveal the test accuracy of post-hoc adjustment, which is searched on a 20\% validation set. The retrain results show the transferability from post-hoc logits adjustment to loss function design. }\label{table:posthoc_supp}\vspace{-20pt}
\end{table}

% \begin{table}
%     \centering
% 	\resizebox{\textwidth}{!}{
% 			\begin{tabular}{lllllll}
% 				\toprule
% \multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{2}{l}{CIFAR100-LT} & \multicolumn{2}{l}{ImageNet-LT} & \multicolumn{2}{l}{CIFAR10-LT+Noise}\\
% \toprule
% \multicolumn{1}{l}{}                  & $\berr$&$\dev$ & $\berr$&$\dev$            & $\berr$&$\dev$          \\
% \midrule
% Cross entropy &  61.94($\pm$0.28)              &    27.13($\pm$0.35)         &  55.52              &   29.06       &43.76($\pm$0.74) & 31.69($\pm$0.81) \\
%  $\nodic_{\text{Bilevel}}$ (AutoBalance \cite{li2021autobalance})     &  56.70($\pm$0.32)              &    20.13($\pm$0.68)         &  50.91              &   26.06      &40.04($\pm$0.79) &   36.30($\pm$0.89)    \\
%  $\name_{\text{Bilevel}}$: $\att_{\text{freq}}$     &  56.64 ($\pm$0.21)             &    19.10($\pm$0.67)         &  50.88              &   24.38       & 39.84($\pm$0.71)&  26.68($\pm$0.86)    \\
%                           $\name_{\text{Bilevel}}$: $\att_{\text{diff}}$     &  58.27($\pm$0.24)              &   \textbf{17.62}($\pm$0.65)             &     53.04  &           \textbf{21.02}         & 40.78($\pm$0.76)&  \textbf{14.31}($\pm$0.82)   \\
%                           $\name_{\text{Bilevel}}$: $\att_{\text{freq}}$+$\att_{\text{diff}}$  &   \textbf{56.38}($\pm$0.19)             &     18.53($\pm$0.63)           &    \textbf{49.32}            &  21.94            & \textbf{38.79}($\pm$0.71)& 20.05($\pm$0.83) \\
% \bottomrule
% 		\end{tabular}}\caption{Standard deviation results of Table~\ref{table:attributes_lt}. Attributes help optimization adapt to dataset heterogeneity. We conduct experiments using bilevel loss design and report the balanced misclassification error,and standard deviation of class-conditional errors with different class-specific attributes.}\label{table:attributes_lt_supp}\vspace{-18pt}

% \end{table}

% 		\begin{table}
% 	\begin{center}\resizebox{\textwidth}{!}{
% 			\begin{tabular}{llllll}
% 				\toprule
% %\multicolumn{1}{l}{} & \multicolumn{4}{l}{Cifar100-LT}  \\
% %\toprule
% \multicolumn{1}{l}{}                  & $\berr$              & $\dev$ & $\cva{0.2}$ &$\quana{0.2}$ &$\werr$ \\
% \midrule
% $\pretrain$&        61.94 ($\pm$0.28)        & 27.13($\pm$0.35)  & 96.95($\pm$0.15)  &  93.01($\pm$0.58) &62.53($\pm$0.53) \\
%   $\nodic_{\text{Post-hoc}}$     &    -1.62($\pm$0.36)            & -8.51($\pm$0.75)   & -11.48($\pm$0.81)  & -12.79($\pm$0.43) &-2.82($\pm$0.56)  \\
%   $\text{LA}_{\text{Post-hoc}}$  &       -3.73($\pm$0.29)        & -8.72($\pm$0.66)   & -12.21($\pm$0.50)  & -15.01($\pm$0.35) &  -3.62($\pm$0.37) \\
%  $\name_{\text{Post-hoc}}$: Single attribute     &    -4.30($\pm$0.26)           & -14.99($\pm$0.21)   & -14.28($\pm$0.92)  & -17.68($\pm$0.12) & -4.03($\pm$0.52)  \\
%  %$\att_{\text{diff}}$    &      -9.38          &  -12.77 & -9.85  & -11.94   \\
%  $\name_{\text{Post-hoc}}$: Combined attributes &  \textbf{-4.36}($\pm$0.25)   &  -13.90($\pm$0.24)  & \textbf{-14.75}($\pm$0.87)  & \textbf{-18.34}($\pm$0.47) & \textbf{-6.21}($\pm$0.49)\\

% \bottomrule
% 		\end{tabular}}\caption{Standard deviation results of Table~\ref{table:attributes_objective}. The error difference between other approaches compared to pre-trained model. The first line shows the performance of Pretrained model, and the following line shows the error difference of other methods (smaller is better). For objectives with $a$, we set $a = 0.2$. This is commly used for difficult or few classes in other papers\cite{zhai2021boosted,liu2019large}. 
% 		%Then the target classes of quantile classes errors and conditional value of errors is the 20th and 0th-20th worst classes. 
% 		For $\dev$, which quantifies the similarly for class-conditional errors, $\quan$ and $\cv$ ,which focus on tail behavior, $\att_{\text{diff}}$ could achieve better result. For weighted test error \eqref{weighted obj}, incorporating weights into CAP leads to significant improvement (results averaged over multiple random weights).
% 		}\label{table:attributes_objective_supp}\vspace{-25pt}
% 	\end{center}
% \end{table}
\begin{table}
    \centering
	\resizebox{\textwidth}{!}{
			\begin{tabular}{lllllll}
				\toprule
\multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{2}{l}{CIFAR100-LT} & \multicolumn{2}{l}{ImageNet-LT} & \multicolumn{2}{l}{CIFAR10-LT+Noise}\\
\toprule
\multicolumn{1}{l}{}                  & $\berr$&$\dev$ & $\berr$&$\dev$            & $\berr$&$\dev$          \\
\midrule
Cross entropy &  61.94($\pm$0.28)              &    27.13($\pm$0.35)         &  55.52              &   29.06       &43.76($\pm$0.74) & 31.69($\pm$0.81) \\
 $\nodic_{\text{Bilevel}}$ (AutoBalance \cite{li2021autobalance})     &  56.70($\pm$0.32)              &    20.13($\pm$0.68)         &  50.91              &   26.06      &40.04($\pm$0.79) &   36.30($\pm$0.89)    \\
 $\name_{\text{Bilevel}}$: $\att_{\text{freq}}$     &  56.64 ($\pm$0.21)             &    19.10($\pm$0.67)         &  50.88              &   24.38       & 39.91($\pm$0.66)&  26.49($\pm$0.80)    \\
                           $\name_{\text{Bilevel}}$: $\att_{\text{diff}}$     &  58.27($\pm$0.24)              &   \textbf{17.62}($\pm$0.65)             &     53.04  &           \textbf{21.02}         & 40.61($\pm$0.61)&  \textbf{14.49}($\pm$0.72)   \\
                           $\name_{\text{Bilevel}}$: $\att_{\text{freq}}$+$\att_{\text{diff}}$  &   \textbf{56.38}($\pm$0.19)             &     18.53($\pm$0.63)           &    \textbf{49.41}($\pm$0.34)            &  22.04($\pm$0.46)            & \textbf{38.36}($\pm$0.79)&
19.78($\pm$0.72) \\
\bottomrule
		\end{tabular}}\caption{Standard deviation results of Table~\ref{table:attributes_lt}. Attributes help optimization adapt to dataset heterogeneity. We conduct experiments using bilevel loss design and report the balanced misclassification error,and standard deviation of class-conditional errors with different class-specific attributes.\xuechen{working on}}\label{table:attributes_lt_supp}\vspace{-18pt}

\end{table}
\input{./update/renew_obj_img}
